Finite-Time Complexity of Online Primal-Dual Natural Actor-Critic Algorithm for Constrained Markov Decision Processes

We consider a discounted cost constrained Markov decision process (CMDP) policy optimization problem, in which an agent seeks to maximize a discounted cumulative reward subject to a number of constraints on discounted cumulative utilities. To solve this constrained optimization program, we study an online actor-critic variant of a classic primal-dual method where the gradients of both the primal and dual functions are estimated using samples from a single trajectory generated by the underlying time-varying Markov processes. This online primal-dual natural actor-critic algorithm maintains and iteratively updates three variables: a dual variable (or Lagrangian multiplier), a primal variable (or actor), and a critic variable used to estimate the gradients of both primal and dual variables. These variables are updated simultaneously but on different time scales (using different step sizes) and they are all intertwined with each other. Our main contribution is to derive a finite-time analysis for the convergence of this algorithm to the global optimum of a CMDP problem. Specifically, we show that with a proper choice of step sizes the optimality gap and constraint violation converge to zero in expectation at a rate $\mathcal{O}(1/K^{1/6})$, where K is the number of iterations. To our knowledge, this paper is the first to study the finite-time complexity of an online primal-dual actor-critic method for solving a CMDP problem. We also validate the effectiveness of this algorithm through numerical simulations.

==> OldFiles/Aug22_AverageReward/introduction.tex <==

\clearpage
We define $A_{L,k}^{\pi}(s, a):=A_{r}^{\pi}(s, a)+\lambda_k A_{g}^{\pi}(s, a)$, and 
\begin{align*}
    \tilde{A}_{L,k}(s,a)= \begin{cases} |\Acal|(\delta_k^r+\lambda_k\delta_k^g), & \text { if } (s_k,a_k)=(s,a) \\ 0, & \text { otherwise }\end{cases}
\end{align*}


Update:
\begin{align}
    \theta_{k+1}(s,a)=\theta_{k}(s,a)+\alpha_k \tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a) \quad \text { or } \quad \pi_{k+1}(a \mid s)=\pi_k(a \mid s) \frac{\exp \left(\alpha_k \tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)}{\tilde{Z}_k(s)}.
\end{align}

Define
\begin{align}
    \tilde{Z}_k(s)=\sum_{a \in \Acal} \pi_k(a \mid s) \exp \left(\alpha_k \tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right).
\end{align}


\begin{align}
& J_{r}(\pi_{k+1})-J_{r}(\pi_k)\notag\\
&= \mathbb{E}_{s \sim \mu_{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[A_{r}^{\pi_k}(s, a)\right] \notag\\
&=\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right]+\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)\right]\notag\\
&\hspace{20pt}-\lambda_k\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) A_{g}^{\pi_{k}}(s, a)\right] \notag\\
&=\frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in A} \pi_{k+1}(a \mid s) \log \left(\frac{\pi_{k+1}(a \mid s)}{\pi_{k}(a \mid s)} \tilde{Z}_k(s)\right)\right]\notag\\
&\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)\right]-\lambda_k\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) A_{g}^{\pi_{k}}(s, a)\right] \notag\\
&=\frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[D_{KL}\left(\pi_{k+1}(\cdot \mid s), \pi_{k}(a \mid s)\right)\right]+ \frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\log\tilde{Z}_k(s))\right]\notag\\
&\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)\right]-\lambda_k\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) A_{g}^{\pi_{k}}(s, a)\right] \notag\\
&\geq \frac{1}{\alpha_k}  \mu_{\pi_{k+1}}(s_k)\left[\log\tilde{Z}_k(s_k))\right]+\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)\right]\notag\\
&\hspace{20pt}-\lambda_k\left(J_{g}(\pi_{k+1})-J_{g}(\pi_k)\right).
\end{align}

Re-arranging the inequality yields
\begin{align}
    &J_{r}(\pi_{k+1})-J_{r}(\pi_k)+\lambda_k\left(J_{g}(\pi_{k+1})-J_{g}(\pi_k)\right)\notag\\
    &\hspace{80pt}\geq \frac{1}{\alpha_k} \mu_{\pi_{k+1}}(s_k)\left[\log\tilde{Z}_k(s))\right]+\mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\sum_{a \in \Acal} \pi_{k+1}(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_{L,k}^{\omega_k,\eta_k}(s, a)\right)\right].
\end{align}


We can show that
\begin{align}
    \log\tilde{Z}_k(s_k)&=\log \left(\sum_{a\in\Acal}\pi_k(a \mid s_k) \exp \left(\alpha_k \tilde{A}_{L,k}^{\omega_k,\eta_k}(s_k, a)\right)\right)\notag\\
    &\geq \sum_{a\in\Acal}\pi_k(a \mid s_k)\log \left( \exp \left(\alpha_k \tilde{A}_{L,k}^{\omega_k,\eta_k}(s_k, a)\right)\right)\notag\\
    &= \alpha_k \sum_{a\in\Acal}\pi_k(a \mid s_k)\tilde{A}_{L,k}^{\omega_k,\eta_k}(s_k, a)\notag\\
    % &= \alpha_k \sum_{a\in\Acal}\pi_k(a \mid s)\left(\delta_k^r+\lambda_k\delta_k^g\right)\notag\\
    &= \alpha_k \sum_{a\in\Acal}\pi_k(a \mid s_k)\left(\tilde{A}_{r,k}^{\omega_k,\eta_k}(s_k, a)-A_r^{\pi_k}(s_k,a)+\lambda_k(\tilde{A}_{g,k}^{\omega_k,\eta_k}(s_k, a)-A_g^{\pi_k}(s_k,a))\right)\notag\\
    &\hspace{20pt}+\alpha_k \sum_{a\in\Acal}\pi_k(a \mid s_k)\left(A_r^{\pi_k}(s_k,a)+\lambda_k A_g^{\pi_k}(s_k,a)\right)\notag\\
    &= \alpha_k \sum_{a\in\Acal}\pi_k(a \mid s_k)\left(\tilde{A}_{r,k}^{\omega_k,\eta_k}(s_k, a)-A_r^{\pi_k}(s_k,a)+\lambda_k(\tilde{A}_{g,k}^{\omega_k,\eta_k}(s_k, a)-A_g^{\pi_k}(s_k,a))\right).
\end{align}

Note that
\begin{align}
    \tilde{A}_{r,k}^{\omega^*(\theta_k),\eta^*(\theta_k)}(s_k,a_k)=|\Acal|A_r^{\pi_k}(s_k,a_k),\quad\text{and}\quad \tilde{A}_{g,k}^{\omega^*(\theta_k),\eta^*(\theta_k)}(s_k,a_k)=|\Acal|A_g^{\pi_k}(s_k,a_k).
\end{align}


Again, from the performance difference lemma, 
\begin{align}
& J_{r}(\pi^*)-J_{r}(\pi_k)\notag\\
&= \mathbb{E}_{s \sim \mu_{\pi^*}, a \sim \pi^*(\cdot \mid s)}\left[A_{r}^{\pi_k}(s, a)\right] \notag\\
&=\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) \tilde{A}_L^{k}(s, a)\right]+\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_L^{k}(s, a)\right)\right]\notag\\
&\hspace{20pt}-\lambda_k\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) A_{g}^{\pi_{k}}(s, a)\right] \notag\\
&=\frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in A} \pi^*(a \mid s) \log \left(\frac{\pi_{k+1}(a \mid s)}{\pi_{k}(a \mid s)} \tilde{Z}_k(s)\right)\right]\notag\\
&\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_L^{k}(s, a)\right)\right]-\lambda_k\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) A_{g}^{\pi_{k}}(s, a)\right] \notag\\
&=\frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi^*}}\left[D_{KL}\left(\pi^*(\cdot \mid s), \pi_{k}(\cdot \mid s)\right)\right]+ \frac{1}{\alpha_k}  \mu_{\pi^*}(s_k)\left[\log\tilde{Z}_k(s_k))\right]\notag\\
&\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi^*}}\left[\sum_{a \in \Acal} \pi^*(a \mid s) \left(A_{L}^{\pi_{k}}(s, a)-\tilde{A}_L^{k}(s, a)\right)\right]-\lambda_k\left(J_g(\pi^*)-J_g(\pi_k)\right).
\end{align}

We assume that for any $\pi$, there exists a constant $C>0$ such that the stationary distribution $\mu_{\pi}(s)>C$ for any $s\in\Scal$. Then,
\begin{align}
    &\frac{1}{\alpha_k} \mu_{\pi^*}(s_k)\left[\log\tilde{Z}_k(s_k)\right]\notag\\
    &=\frac{1}{\alpha_k} \mathbb{E}_{s \sim \mu_{\pi^*}}\left[\log\tilde{Z}_k(s)-\left(\alpha_k \sum_{a\in\Acal}\pi_k(a \mid s)\left(\tilde{A}_{r,k}(s, a)-A_r^{\pi_k}(a\mid s)+\lambda_k(\tilde{A}_{g,k}(s, a)-A_g^{\pi_k}(a\mid s))\right)\right)\right]\notag\\
    &\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi^*}}\left[ \sum_{a\in\Acal}\pi_k(a \mid s)\left(\tilde{A}_{r,k}(s, a)-A_r^{\pi_k}(a\mid s)+\lambda_k(\tilde{A}_{g,k}(s, a)-A_g^{\pi_k}(a\mid s))\right)\right]\notag\\
    &\leq \frac{1}{\alpha_k C} \mathbb{E}_{s \sim \mu_{\pi_{k+1}}}\left[\log\tilde{Z}_k(s)-\left(\alpha_k \sum_{a\in\Acal}\pi_k(a \mid s)\left(\tilde{A}_{r,k}(s, a)-A_r^{\pi_k}(a\mid s)+\lambda_k(\tilde{A}_{g,k}(s, a)-A_g^{\pi_k}(a\mid s))\right)\right)\right]\notag\\
    &\hspace{20pt}+\mathbb{E}_{s \sim \mu_{\pi^*}}\left[ \sum_{a\in\Acal}\pi_k(a \mid s)\left(\tilde{A}_{r,k}(s, a)-A_r^{\pi_k}(a\mid s)+\lambda_k(\tilde{A}_{g,k}(s, a)-A_g^{\pi_k}(a\mid s))\right)\right]
\end{align}

==> OldFiles/Oct11_MainTheoremProof/MainResults.tex <==
\section{Main Results}\label{sec:mainresults}

This section presents our finite-time analysis of Algorithm~\ref{Alg:AC} and highlights the main technical difficulty. In Section~\ref{sec:mainresults:convergence_rate}, we state our main theorem, which characterizes the convergence of the actor to the global optimality of \eqref{eq:objective} in both the objective function and constraint violation, under challenges caused by the coupled multi-time-scale updates and the time-varying Markovian samples. In Section~\ref{sec:mainresults:challenges}, we discuss these challenges in details, sketch our approach to treat the problem, and introduce preliminary results on the convergence of the dual variable, actor, and critic as coupled functions of each other. Finally, we
% use the preliminary results to
provide the proof of the main theorem in Section~\ref{sec:mainresults:proof_theorem}.


\subsection{Finite-Time Convergence}\label{sec:mainresults:convergence_rate}

We start by defining the mixing time of a Markov chain $\{X_k\}$, which measures the time for $\{X_k\}$ to approach its stationary distribution \citep{LevinPeresWilmer2006}. 
\begin{definition}\label{def:mixing_time}
Let $\mu$ denote the stationary distribution of the Markov chain $\{X_k\}$.
For any scalar $c>0$, the mixing time of the Markov chain $\{X_k\}$ associated with $c$ is defined as
\[\tau(c) \hspace{-2pt}=\hspace{-2pt} \min\{k\hspace{-2pt}\geq\hspace{-2pt} 0\hspace{-2pt}:\hspace{-2pt}\sup_{X\in\Xcal}\hspace{-2pt}d_{\text{TV}}(\hspace{-1pt}P(X_k=\hspace{-2pt}\cdot\hspace{-2pt}\,|X_0\hspace{-2pt}=\hspace{-2pt}X\hspace{-1pt}),\mu(\cdot))\leq c\}.\]
\end{definition}
We consider the following assumption on the Markov chain generated by the transition probability $P^{\pi}(s' \mid s)=\sum_{a\in\Acal}\Pcal(s'\mid s,a)\pi(a\mid s)$ under the policy $\pi$, which basically says that it mixes geometrically fast.
\begin{assump}\label{assump:markov-chain}
Given any $\theta$, the Markov chain $\{X_{k}\}$ generated by $P^{\pi}$ has a unique stationary distribution $\mu_{\pi}$, and is uniformly geometrically ergodic, i.e., there exist $C_{0}\geq 1$ and $\rho\in (0,1)$ such that
\begin{equation*}
\sup_{X\in\Xcal}d_{\text{TV}}(P^{\pi}(X_k=\cdot \mid X_0=X),\mu_{\pi}(\cdot))\hspace{-2pt}\leq\hspace{-2pt} C_{0}\rho^k,\, \forall k\geq 0.
\end{equation*}
\end{assump}
This assumption is standard in the study of MDP \citep{chen2019finite,zeng2020finite} and implies that there exists a positive constant $C$ such that 
\begin{equation}
\tau(c) \leq C\ln\left(1/c\right)\quad\forall c.\label{eq:mixing:tau}
\end{equation} 
In this work, we denote $\tau\triangleq\tau(\alpha)$, where $\alpha$ is the step size for the actor update.


\begin{thm}\label{thm:main}
Let the step size sequences be
\begin{align*}
    \eta=\frac{\eta_0}{K^{5/6}},\quad\alpha=\frac{\alpha_0}{K^{5/6}},\quad \beta=\frac{\beta_0}{K^{1/2}},\quad \epsilon=\frac{\epsilon_0}{K^{1/6}}
\end{align*}
such that $\frac{(1-\gamma)\mu\epsilon\beta}{|\Acal|}\leq 1$. Then, under Assumption~\ref{assump:Slater} and \ref{assump:markov-chain}, we have
\end{thm}


\subsection{Technical Challenges \& Solution Sketch}\label{sec:mainresults:challenges}

The first main technical challenge of the work stems from the Markovian samples. To deal with the noise of the dependent samples from a time-invariant Markov chain, one can utilize the fast mixing time afforded by Assumption~\ref{assump:markov-chain} to show that the noise decays geometrically fast \citep{srikant2019finite,doan2020finite}. However, such analysis is not directly applicable to this work as the samples of our algorithm are from a time-varying Markov chain generated by the ever-changing behavior policy as illustrated below
\begin{align*}
    (s_0,a_0) \stackrel{\Pcal,\widehat{\pi}_{0}}{\longrightarrow} (s_1,a_1) \stackrel{\Pcal,\widehat{\pi}_{1}}{\longrightarrow} (s_2,a_2) \stackrel{\Pcal,\widehat{\pi}_{2}}{\longrightarrow} \hspace{-2pt}\cdots\hspace{-3pt} \stackrel{\Pcal,\widehat{\pi}_{k-1}}{\longrightarrow} (s_{k},a_{k}),
\end{align*}
which implies that the stationary distribution of this Markov chain changes with $\widehat{\pi}_k$ over time, and the noise caused by samples from this chain requires special treatment. In our analysis, we will show that the shift of the stationary distribution is controlled by the shift of the behavior policy, which can be properly bounded with the correct step size choice.


Another challenge of this work is due to the multi-time-scale nature of the updates. Recall that Algorithm~\ref{Alg:AC} uses four step size parameters, namely, the actor step size $\alpha$, the critic step size $\beta$, the dual variable step size $\eta$, and the exploration parameter $\epsilon$. \citet{borkar2005actor} shows that the relative order $\eta\leq\alpha\leq\beta\leq\epsilon$ leads to the asymptotic convergence of the algorithm, but the exact choice of the parameters as a function of the horizon $K$ that yields a finite-time convergence rate remains unknown. In this work, we fill in this gap by properly selecting and balancing the step sizes through a four-time-scale analysis. Compared with the existing works in two-time-scale stochastic approximation/optimization \citep{doan2020nonlinear,hong2020two,zeng2021two} and analysis of actor-critic algorithms involving up to three time scales \citep{wu2020finite,khodadadian2021finite}, the additional time scale(s) of this work further complicates the analysis.

In addition, we note that the time-varying Markov chain above also reveals the deep dependency of the variables on each other. The updates of the critic and dual variable depend on samples generated by the $\epsilon$-exploration version of previous actor policies $\{\widehat{\pi}_t\}_{t\leq k-1}$ and in turn affect the actor update in the next iteration. A similar interaction also exists between the dual variable and the critic. Combined with the effect of multiple time scales, the variable coupling further creates increased difficulty of characterizing the convergence of each variable individually.



% In addition, the heavily coupled updates in \eqref{Alg:AC:sample}-\eqref{Alg:AC:dual_update} create a deep dependency of the variables on each other. Consider, for example, the critic $\widehat{Q}_{i,k}$, which is used to learn the actor $\pi_{k}$ 
% and the dual variable $\lambda_k$ 
% but also depends on samples generated under the $\epsilon$-exploration version of previous actor policy $\{\widehat{\pi}_t\}_{t\leq k-1}$. 
% Similar interactions also exist between the actor and the dual variable, and between the dual variable and the critic.

Our approach to handle the intertwined system of variables is to choose a proper decoupling scheme according to the structure of the updates. We observe that only the update of the critic variable in \eqref{Alg:AC:critic_update} directly utilizes the samples. The effect of the samples on the actor and dual variable is indirect through the critic. This motivates us to separate the analysis of the actor and dual variable from that of the critic. Specifically, we aim to establish 1) the convergence of the actor and the dual variable up to errors that depend on the accuracy of the critic and 2) the convergence of the critic as a function of the distribution shift of the Markovian samples, which can be further traced back to depend on the one-step drift of the actor.

\noindent\textbf{Convergence of Actor and Dual:} Since the actor and dual variable updates do not explicitly depend on the samples, we can avoid dealing with the complications arising from the Markovian samples in this part of the analysis. For now, we only focus on the convergence of actor and the dual variable by deriving the convergence of the objective function and constraint violation up to an error that scales with the inaccuracy of the critic variable. 
\begin{prop}\label{prop:convergence_obj_constraintviolation}
Under Assumption~\ref{assump:Slater}, the iterates of the actor $\{\pi_k\}$ converges to attain the optimal objective function value
% \noindent\textbf{Objective function:}
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)\right)\hspace{-2pt}\leq\hspace{-2pt} \frac{\log|\Acal|}{(1-\gamma)K\alpha}\hspace{-2pt}+\hspace{-2pt}\frac{6N}{\xi(1-\gamma)^3 K}&\notag\\
    + \frac{2N\eta}{(1-\gamma)^2}+\frac{D_2}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|.&
\end{align*}
Furthermore, $\{\pi_k\}$ also converges in constraint violation
\begin{align*}
    &\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\Big[b_i-V_{i}^{\pi_k}(\rho)\Big]_{+}\notag\\
    &\leq \frac{\xi(1-\gamma)}{2}\Big(\frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}\notag\\
    &\hspace{20pt}+\frac{8N}{K\eta\xi^2(1-\gamma)^2}+\frac{D_2}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|\Big),
\end{align*}
where $D_2=\frac{4(2-\gamma)}{\xi(1-\gamma)^3}+\frac{4}{\xi(1-\gamma)}$.
\end{prop}

Due to the space limit, we delay the proof of the proposition to the supplementary material. If the estimates of the critic were exactly correct, i.e. $\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|=0$, we would obtain $\Ocal(1/\sqrt{K})$ convergence for both the objective function and constraint violation by choosing $\eta=\Ocal(1/\sqrt{K})$ and $\alpha=\Ocal(1)$, which recovers the convergence rate of the natural policy gradient method in \citet{ding2020natural}. In this work, such step size choices are not possible due to the presence of the critic error and the restrictions on the step sizes.


\noindent\textbf{Convergence of Critic:} We now establish the convergence of the critic to the true value function of the behavior policy, i.e. defining 
\begin{align}
    z_{i,k}=\widehat{Q}_{i,k}-Q_i^{\widehat{\pi}_k}\in\mathbb{R}^{|\Scal||\Acal|},\label{eq:def_z}
\end{align}
we aim to bound $\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|^2$.

As we have discussed earlier in this section, the coupling between the variables creates a dependency of the critic convergence on the step-wise drifts of the actor. We remove such dependency by choosing the step sizes such that the critic updates on a much faster time scale than the actor does. This essentially makes the drifts of the actor insignificant from the eye of the critic and reduces the bound on $\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|^2$ to only depend on the ratio of the step sizes.





\begin{prop}\label{prop:conv_critic}
Under Assumption \ref{assump:markov-chain}, if step sizes observe
\[\frac{(1-\gamma)\mu\epsilon\beta}{|\Acal|}\leq 1\]
then the iterates $\{\widehat{Q}_{i,k}\}$ and $\{\widehat{\pi}_{k}\}$ satisfy
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|^2\leq \frac{8|\Scal||\Acal|^2 \tau}{(1-\gamma)^3\mu\epsilon\beta K}+\frac{D_1 N^2|\Acal|}{(1-\gamma)\mu}\frac{\beta\tau^2}{\epsilon}&\notag\\
    +\frac{9|\Scal|^2|\Acal|^5 N^2 \alpha^2}{\xi\mu^2 (1-\gamma)^9 \epsilon^2 \beta^2}&,
\end{align*}
where the constants are
\begin{align*}
    &C_1\hspace{-3pt}=\hspace{-3pt}\frac{2\sqrt{2}(|\Scal|\Acal|)^{3/2}}{(1-\gamma)^3}\hspace{-2pt}+\hspace{-2pt}\frac{8|\Scal|^2|\Acal|^3}{(1-\gamma)^2}\hspace{-1pt}\big(\hspace{-2pt}\left\lceil\log _{\rho} m^{-1}\hspace{-1pt}\right\rceil\hspace{-2pt}+\hspace{-2pt}\frac{1}{1\hspace{-2pt}-\hspace{-2pt}\rho}\hspace{-2pt}+\hspace{-2pt}2\big)\hspace{-1pt},\\
    &C_2\hspace{-3pt}=\hspace{-3pt}1\hspace{-2pt}+\hspace{-2pt}\frac{9\sqrt{2|\Scal||\Acal|}}{1-\gamma},\quad C_3\hspace{-3pt}=\hspace{-3pt}\frac{4|\Scal|^{3/2}|\Acal|^{3/2}}{1-\gamma}(1\hspace{-2pt}+\hspace{-2pt}\frac{3|\Scal||\Acal|}{1-\gamma}),\\
    &D_1\hspace{-3pt}=\hspace{-3pt}\frac{2(3C_1+6C_2+4C_3) (|\Scal||\Acal|)^{3/2} }{\xi^{1/2} (1-\gamma)^{7/2}}+\frac{36 (|\Scal||\Acal|)^3}{\xi(1-\gamma)^7}.
\end{align*}
\end{prop}

With its detailed proof presented in the supplementary material, this proposition relies on the fast mixing time of the Markov chain under all behavior policy iterates $\{\widehat{\pi}_k\}$ and the slow drift of the actor compared with the critic. We note that the critic learns the Q function of the behavior policy rather than that of the actor policy which we need to use in combination with Proposition~\ref{prop:convergence_obj_constraintviolation}, but the distance between the behavior policy and the actor policy can be properly controlled by choosing the parameter $\epsilon$.



\subsection{Proof of Theorem~\ref{thm:main}}\label{sec:mainresults:proof_theorem}
In this section, we provide a proof of our main theorem using intermediate results established in Proposition~\ref{prop:convergence_obj_constraintviolation} and \ref{prop:conv_critic}. We first introduce the following lemma on the Lipschitz continuity of the Q function with respect to the policy.
\begin{lem}[\citet{khodadadian2021finite} Lemma 8]\label{lem:Q_Lipschitz_pi}
    For any policy $\pi_1$, $\pi_2$, we have
    \begin{align*}
        \|Q_i^{\pi_1}-Q_i^{\pi_2}\|\leq L_Q\|\pi_1-\pi_2\|,
    \end{align*}
    where $L_Q=\frac{|\Scal||\Acal|}{(1-\gamma)^2}$.
\end{lem}



By Proposition~\ref{prop:conv_critic} and the Cauchy-Schwarz inequality, 
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|\leq \left(\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|^2\right)^{1/2}\notag\\
    &\leq \Big(\frac{8|\Scal||\Acal|^2 \tau}{(1-\gamma)^3\mu\epsilon\beta K}+\frac{D_1 N^2|\Acal|}{(1-\gamma)\mu}\frac{\beta\tau^2}{\epsilon}\notag\\
    &\hspace{20pt}+\frac{9|\Scal|^2|\Acal|^5 N^2 \alpha^2}{\xi\mu^2 (1-\gamma)^9 \epsilon^2 \beta^2}\Big)^{1/2}\notag\\
    &\leq \frac{3|\Scal|^{1/2}|\Acal|}{(1-\gamma)^{3/2}\mu^{1/2}}\frac{1}{\epsilon^{1/2}\beta^{1/2} K^{1/2}}+\frac{D_1^{1/2} N|\Acal|^{1/2}}{(1-\gamma)^{1/2}\mu^{1/2}}\frac{\beta^{1/2}\tau}{\epsilon^{1/2}}\notag\\
    &\hspace{20pt}+\frac{3|\Scal||\Acal|^{5/2} N}{\xi^{1/2}\mu (1-\gamma)^{9/2}}\frac{\alpha}{\epsilon\beta}
    \label{thm:main:eq2}
\end{align}


The bounds in Proposition \ref{prop:convergence_obj_constraintviolation} depend on the error $\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|$, which we decompose and bound using \eqref{thm:main:eq2}. From the definition of $z_{i,k}$ in \eqref{eq:def_z}, we have for any $i=0,1,\cdots,N$
\begin{align*}
    &\frac{1}{K}\sum_{k=0}^{K-1}\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\|\notag\\
    &\leq \frac{1}{K}\sum_{k=0}^{K-1}\|Q_{i}^{\widehat{\pi}_k}-Q_{i}^{\pi_k}\|+\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|\notag\\
    &\leq \frac{1}{K}\sum_{k=0}^{K-1}\frac{|\Scal||\Acal|}{(1-\gamma)^2}\|\widehat{\pi}_k-\pi_k\|+\frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|\notag\\
    &\leq \frac{2|\Scal|^{3/2}|\Acal| \epsilon}{(1-\gamma)^2}+\frac{3|\Scal|^{1/2}|\Acal|}{(1-\gamma)^{3/2}\mu^{1/2}}\frac{1}{\epsilon^{1/2}\beta^{1/2} K^{1/2}}\notag\\
    &\hspace{20pt}+\frac{D_1^{1/2} N|\Acal|^{1/2}}{(1-\gamma)^{1/2}\mu^{1/2}}\frac{\beta^{1/2}\tau}{\epsilon^{1/2}}+\frac{3|\Scal||\Acal|^{5/2} N}{\xi^{1/2}\mu (1-\gamma)^{9/2}}\frac{\alpha}{\epsilon\beta},
\end{align*}
where the second inequality uses Lemma \ref{lem:Q_Lipschitz_pi}, and the third inequality follows from \eqref{thm:main:eq2} and
\begin{align*}
    &\|\widehat{\pi}_k-\pi_k\|=\|\frac{\epsilon}{|\Acal|}\1_{|\Scal||\Acal|}+(1-\epsilon)\pi_k-\pi_k\|\notag\\
    &\leq\epsilon\|\frac{1}{|\Acal|}\1_{|\Scal||\Acal|}\|+\epsilon\|\pi_k\|\leq \epsilon\frac{|\Scal|^{1/2}}{|\Acal|^{1/2}}+\epsilon|\Scal|^{1/2}\hspace{-2pt}\leq\hspace{-2pt}2\epsilon|\Scal|^{1/2}.
\end{align*}

Using the bound above in Proposition \ref{prop:convergence_obj_constraintviolation}, we have
\begin{align*}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)\right)\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+ \frac{2N\eta}{(1-\gamma)^2}\notag\\
    &\hspace{20pt}+\frac{D_2}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\| \notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+ \frac{2N\eta}{(1-\gamma)^2}\notag\\
    &\hspace{20pt}+D_2\Big(\frac{2|\Scal|^{3/2}|\Acal| \epsilon}{(1-\gamma)^2}+\frac{3|\Scal|^{1/2}|\Acal|}{(1-\gamma)^{3/2}\mu^{1/2}}\frac{1}{\epsilon^{1/2}\beta^{1/2} K^{1/2}}\notag\\
    &\hspace{20pt}+\frac{D_1^{1/2} N|\Acal|^{1/2}}{(1-\gamma)^{1/2}\mu^{1/2}}\frac{\beta^{1/2}\tau}{\epsilon^{1/2}}+\frac{3|\Scal||\Acal|^{5/2} N}{\xi^{1/2}\mu (1-\gamma)^{9/2}}\frac{\alpha}{\epsilon\beta}\Big)
\end{align*}

For the constraint violation,
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\Big[b_i-V_{i}^{\pi_k}(\rho)\Big]_{+}\notag\\
    &\leq\frac{\xi(1-\gamma)}{2}\Big(\frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}\notag\\
    &\hspace{20pt}+\frac{8N}{K\eta\xi^2(1-\gamma)^2}+\frac{D_2}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|\Big)\notag\\
    &\leq \frac{\xi(1-\gamma)}{2}\Big(\frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{8N}{K\eta\xi^2(1-\gamma)^2}\notag\\
    &\hspace{20pt}+D_2\Big(\frac{2|\Scal|^{3/2}|\Acal| \epsilon}{(1-\gamma)^2}+\frac{3|\Scal|^{1/2}|\Acal|}{(1-\gamma)^{3/2}\mu^{1/2}}\frac{1}{\epsilon^{1/2}\beta^{1/2} K^{1/2}}\notag\\
    &\hspace{20pt}+\frac{D_1^{1/2} N|\Acal|^{1/2}}{(1-\gamma)^{1/2}\mu^{1/2}}\frac{\beta^{1/2}\tau}{\epsilon^{1/2}}+\frac{3|\Scal||\Acal|^{5/2} N}{\xi^{1/2}\mu (1-\gamma)^{9/2}}\frac{\alpha}{\epsilon\beta}\Big)\Big)
\end{align}




==> OldFiles/Oct19_Proofs/Proof_Lemma.tex <==

\section{Proof of Technical Lemmas}

% \subsection{Proof of Lemma \ref{lem:strong_duality}}

% It is known that the strong duality holds if the Slater's condition holds and the perturbation function $P(\phi)$ is concave (see \citet{rockafellar1970convex}[Cor. 30.2.2] and \citet{paternain2019constrained}[Proposition 1]).

% We assume the Slater's condition in Assumption \ref{assump:Slater} and have established the concavity of the perturbation function is Lemma \ref{lem:perturbation_concave}. As a result, we conclude that the strong duality holds.

% \qed

\subsection{Proof of Lemma \ref{lem:hatpi_onestepdrift}}
We have
\begin{align*}
    \|\widehat{\pi}_{k+1}-\widehat{\pi}_{k}\|\leq \|\pi_{k+1}-\pi_{k}\|\leq \|\theta_{k+1}-\theta_{k}\|
\end{align*}
where the second inequality is obvious from the definition of the behavior policy in \eqref{Alg:AC:behaviorpolicy_update}, and the third inequality is due to the softmax function being Lipschitz with constant 1.

From the update rule \eqref{Alg:AC:actor_update}, we have
\begin{align*}
    \|\theta_{k+1}-\theta_{k}\|^2 &= \alpha^2\|\widehat{Q}_{0,k}+\lambda_k^{\top} \widehat{Q}_{g,k}\|^2\leq 2\alpha^2\|\widehat{Q}_{0,k}\|^2+2\alpha^2\|\lambda_k^{\top} \widehat{Q}_{g,k}\|^2\notag\\
    &\leq 2\alpha^2\|\widehat{Q}_{0,k}\|^2+2\alpha^2 N\sum_{i=1}^{N}|\lambda_i|\| \widehat{Q}_{i,k}\|^2 \leq 2\alpha^2\frac{|\Scal||\Acal|}{(1-\gamma)^2}+\frac{4\alpha^2 N}{\xi(1-\gamma)}\sum_{i=1}^{N}\frac{|\Scal||\Acal|}{(1-\gamma)^2}\notag\\
    &\leq \frac{6\alpha^2 N^2 |\Scal||\Acal|}{\xi(1-\gamma)^3}.
\end{align*}

Combining the two inequalities above, we have
\begin{align*}
    \|\widehat{\pi}_{k+1}-\widehat{\pi}_{k}\|\leq \frac{3(|\Scal||\Acal|)^{1/2} N \alpha}{\xi^{1/2}(1-\gamma)^{3/2}}.
\end{align*}


\qed



\subsection{Proof of Lemma \ref{lem:z_onestepdrift}}
\begin{align*}
    \|z_{i,k+1}-z_{i,k}\|^2&=\|\widehat{Q}_{i,k+1}-Q_i^{\widehat{\pi}_{k+1}}-\widehat{Q}_{i,k}+Q_i^{\widehat{\pi}_{k}}\|^2\leq 2\|\widehat{Q}_{i,k+1}-\widehat{Q}_{i,k}\|^2+2\|Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}}\|^2\notag\\
    &\leq 2\beta^2(\frac{2}{1-\gamma}+1)^2+2\|Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}}\|^2 \leq 2\beta^2(\frac{2}{1-\gamma}+1)^2+\frac{18\gamma^2 (|\Scal||\Acal|)^3 N^2 \alpha^2}{\xi(1-\gamma)^7}\notag\\
    &\leq \frac{36 (|\Scal||\Acal|)^3 N^2 \beta^2}{\xi(1-\gamma)^7},
\end{align*}
where the second inequality comes from the update \eqref{Alg:AC:critic_update}, the third inequality applies Lemma \ref{lem:Q_Lipschitz_pi} and \ref{lem:hatpi_onestepdrift}, and the last inequality combines terms using $\alpha\leq\beta$.

Taking the square root yields
\begin{align*}
    \|z_{i,k+1}-z_{i,k}\|&\leq \frac{6 (|\Scal||\Acal|)^{3/2} N \beta}{\xi^{1/2}(1-\gamma)^{7/2}}.
\end{align*}

\qed


\subsection{Proof of Lemma \ref{lem:bound_Gamma}}
% Defining the terms
% \begin{align*}
%     &T_1=z_{i,k}^{\top}(M(O_k)(Q_i^{\widehat{\pi}_k}-Q_i^{\widehat{\pi}_{k-\tau}}))+z_{i,k}^{\top}(\widebar{M}^{\widehat{\pi}_{k-\tau}}-\widebar{M}^{\widehat{\pi}_{k}})z_{i,k}\\
%     &T_2=(z_{i,k}-z_{i,k-\tau})^{\top}(R_i(O_k)+M(O_k)Q_i^{\widehat{\pi}_{k-\tau}})+z_{i,k}^{\top}(M(O_k)-\widebar{M}^{\widehat{\pi}_{k-\tau}})z_{i,k}-z_{i,k-\tau}^{\top}(M(O_k)-\widebar{M}^{\widehat{\pi}_{k-\tau}})z_{i,k-\tau}\\
%     &T_3=
% \end{align*}


We introduce the following auxiliary Markov chain of states and actions generated under the policy $\theta_{k-\tau}$ starting from $s_{k-\tau}$ as follows
\begin{align}
&{s}_{k-\tau} \stackrel{\widehat{\pi}_{k-\tau-1}}{\longrightarrow}  \widetilde{a}_{k-\tau}\stackrel{\Pcal}{\longrightarrow}  \widetilde{s}_{k-\tau+1} \stackrel{\widehat{\pi}_{k-\tau-1}}{\longrightarrow} a_{k-\tau+1}\stackrel{\Pcal}{\longrightarrow}  \cdots\stackrel{\Pcal}{\longrightarrow}\widetilde{s}_{k} \stackrel{\widehat{\pi}_{k-\tau-1}}{\longrightarrow}  \widetilde{a}_{k}\stackrel{\Pcal}{\longrightarrow}  \widetilde{s}_{k+1} \stackrel{\widehat{\pi}_{k-\tau-1}}{\longrightarrow}  \widetilde{a}_{k+1}.
\label{eq:def_auxiliaryMarkovChain}
\end{align}
% and we use $d_k$ to denote the distribution of $\widetilde{X}_{k}$. 
For clarity, we recall that the original Markovian samples generated by our algorithm are
\begin{align*}
&{s}_{k-\tau} \stackrel{\widehat{\pi}_{k-\tau-1}}{\longrightarrow}  a_{k-\tau}\stackrel{\Pcal}{\longrightarrow}  s_{k-\tau+1} \stackrel{\widehat{\pi}_{k-\tau}}{\longrightarrow} a_{k-\tau+1}\stackrel{\Pcal}{\longrightarrow}  \cdots\stackrel{\Pcal}{\longrightarrow} s_{k} \stackrel{\widehat{\pi}_{k-1}}{\longrightarrow}  a_{k}\stackrel{\Pcal}{\longrightarrow}  s_{k+1} \stackrel{\widehat{\pi}_{k}}{\longrightarrow}  a_{k+1}.
\end{align*}

We can decompose the term of interest
\begin{align}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)]&=\mathbb{E}[\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k},O_k)]\notag\\
    &\hspace{20pt}+\mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},O_k)]\notag\\
    &\hspace{20pt}+\mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},\widetilde{O}_k)]\notag\\
    &\hspace{20pt}+\mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},\widetilde{O}_k)]
    \label{lem:bound_Gamma_decomposition}
\end{align}


We introduce the following lemmas to bound each term of \eqref{lem:bound_Gamma_decomposition}.

\begin{lem}\label{lem:Gamma_bound:lem1}
We have for all $\pi_1$, $\pi_2$, $z$, $O$
\begin{align*}
    \Gamma_i(\pi_1,z,O)-\Gamma_i(\pi_2,z,O)\leq C_2\|\pi_1-\pi_2\|,
\end{align*}
where $C_2=\frac{2\sqrt{2}|\Scal|^{3/2}|\Acal|^{3/2}}{(1-\gamma)^3}+\frac{8|\Scal|^2|\Acal|^3}{(1-\gamma)^2}\left(\left\lceil\log _{\rho} m^{-1}\right\rceil+\frac{1}{1-\rho}+2\right)$.
% $C_2=\frac{2\sqrt{2|\Scal||\Acal|}L_Q}{1-\gamma}+\frac{8|\Scal|^2|\Acal|^3}{(1-\gamma)^2}\left(\left\lceil\log _{\rho} m^{-1}\right\rceil+\frac{1}{1-\rho}+2\right)=\frac{2\sqrt{2}|\Scal|^{3/2}|\Acal|^{3/2}}{(1-\gamma)^3}+\frac{8|\Scal|^2|\Acal|^3}{(1-\gamma)^2}\left(\left\lceil\log _{\rho} m^{-1}\right\rceil+\frac{1}{1-\rho}+2\right)$.

(This is \citet{khodadadian2021finite}[Lemma 11].)
\end{lem}

\begin{lem}\label{lem:Gamma_bound:lem2}
We have for all $\pi$, $z_1$, $z_2$, $O$
\begin{align*}
    \Gamma_i(\pi,z_1,O)-\Gamma_i(\pi,z_2,O)\leq C_3\|z_1-z_2\|,
\end{align*}
where $C_3=1+\frac{9\sqrt{2|\Scal||\Acal|}}{1-\gamma}$.

(This is \citet{khodadadian2021finite}[Lemma 12].)
\end{lem}



\begin{lem}\label{lem:Gamma_bound:lem3}
Defining $\Fcal_{t-\tau}=\{s_{t-\tau},\widehat{\pi}_{k-\tau-1},z_{i,k-\tau}\}$, we have
\begin{align*}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau-1},z_{i,k-\tau},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau-1},z_{i,k-\tau},\widetilde{O}_k)\mid F_{k-\tau}]\leq C_4\sum_{t=k-\tau}^{k}\mathbb{E}[\|\widehat{\pi}_{t}-\widehat{\pi}_{k-\tau-1}\|\mid F_{k-\tau}],
\end{align*}
where $C_4=\frac{4|\Scal|^{3/2}|\Acal|^{3/2}}{1-\gamma}(1+\frac{3|\Scal||\Acal|}{1-\gamma})$.

(This is \citet{khodadadian2021finite}[Lemma 13].)
\end{lem}





\begin{lem}\label{lem:Gamma_bound:lem4}
Defining $\Fcal_{t-\tau}=\{s_{t-\tau},\widehat{\pi}_{k-\tau-1},z_{i,k-\tau}\}$, we have
\begin{align*}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau-1},z_{i,k-\tau},\widetilde{O}_k)\mid F_{k-\tau}]\leq C_4\alpha.
\end{align*}

(This is \citet{khodadadian2021finite}[Lemma 14].)
\end{lem}


Lemma \ref{lem:Gamma_bound:lem1} implies that the first term of \eqref{lem:bound_Gamma_decomposition} can be bounded as
\begin{align}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k},O_k)]&\leq C_2\mathbb{E}[\|\widehat{\pi}_k-\widehat{\pi}_{k-\tau}\|]\leq C_2\sum_{t=k-\tau}^{k-1}\mathbb{E}[\|\widehat{\pi}_{t+1}-\widehat{\pi}_{t}\|] \notag\\
    &\leq C_2 \sum_{t=k-\tau}^{k-1} \frac{3(|\Scal||\Acal|)^{1/2} N \alpha}{\xi^{1/2}(1-\gamma)^{3/2}}\leq \frac{3C_2(|\Scal||\Acal|)^{1/2} N \alpha\tau}{\xi^{1/2}(1-\gamma)^{3/2}},
    \label{lem:bound_Gamma:term1}
\end{align}
where the third inequality uses Lemma \ref{lem:hatpi_onestepdrift}.

Similarly, applying Lemma \ref{lem:Gamma_bound:lem2}, we consider the second term of \eqref{lem:bound_Gamma_decomposition}
\begin{align}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},O_k)]&\leq C_3 \mathbb{E}[\|z_{i,k}-z_{i,k-\tau}\|]\notag\\
    &\hspace{-200pt}\leq C_3\sum_{t=k-\tau}^{k-1}\mathbb{E}[\|z_{i,t+1}-z_{i,t}\|]\leq C_3\sum_{t=k-\tau}^{k-1}\frac{6 (|\Scal||\Acal|)^{3/2} N \beta}{\xi^{1/2}(1-\gamma)^{7/2}}\leq \frac{6C_3 (|\Scal||\Acal|)^{3/2} N \beta\tau}{\xi^{1/2}(1-\gamma)^{7/2}}.
    \label{lem:bound_Gamma:term2}
\end{align}


Using Lemma \ref{lem:Gamma_bound:lem3} and taking the expectation over $\Fcal_{k-\tau}$, we have for the following bound on the third term of \eqref{lem:bound_Gamma_decomposition},
\begin{align}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},O_k)-\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},\widetilde{O}_k)]&\leq C_4 \sum_{t=k-\tau}^{k}\mathbb{E}[\|\widehat{\pi}_{t}-\widehat{\pi}_{k-\tau-1}\|]\notag\\
    &\hspace{-200pt}\leq C_4\sum_{t=k-\tau}^{k}\tau\frac{3(|\Scal||\Acal|)^{1/2} N \alpha}{\xi^{1/2}(1-\gamma)^{3/2}}=\frac{3C_4(|\Scal||\Acal|)^{1/2} N \alpha\tau^2}{\xi^{1/2}(1-\gamma)^{3/2}},
    \label{lem:bound_Gamma:term3}
\end{align}
where the second inequality follows from Lemma \ref{lem:hatpi_onestepdrift}.

The fourth term of \eqref{lem:bound_Gamma_decomposition} follows similarly from taking the expectation over $\Fcal_{k-\tau}$ on the result of Lemma \ref{lem:Gamma_bound:lem4}
\begin{align}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_{k-\tau},z_{i,k-\tau},\widetilde{O}_k)]\leq C_4\alpha
    \label{lem:bound_Gamma:term4}
\end{align}

Using \eqref{lem:bound_Gamma:term1}-\eqref{lem:bound_Gamma:term4} in \eqref{lem:bound_Gamma_decomposition}, we have
\begin{align*}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)] &\leq \frac{3C_2(|\Scal||\Acal|)^{1/2} N \alpha\tau}{\xi^{1/2}(1-\gamma)^{3/2}}+ \frac{6C_3 (|\Scal||\Acal|)^{3/2} N \beta\tau}{\xi^{1/2}(1-\gamma)^{7/2}}\notag\\
    &\hspace{20pt}+\frac{3C_4(|\Scal||\Acal|)^{1/2} N \alpha\tau^2}{\xi^{1/2}(1-\gamma)^{3/2}}+C_4\alpha\notag\\
    &\leq \frac{(3C_2+6C_3+4C_4) (|\Scal||\Acal|)^{3/2} N \beta\tau^2}{\xi^{1/2}(1-\gamma)^{7/2}},
\end{align*}
where in the last inequality we combine terms using $|\Scal||\Acal|\geq 1$, $N\geq 1$, $\xi\leq 1$, and $\alpha\leq\beta$.

\qed



\subsection{Proof of Lemma \ref{lem:perturbation_concave}}

Given any $\phi_1,\phi_2\in\mathbb{R}^{N}$, we use $\pi_1$ and $\pi_2$ to denote the policy that attains $P(\phi_1)$ and $P(\phi_2)$, respectively. We want to show that for any $a\in[0,1]$
\begin{align}
    P(a\phi_1+(1-a)\phi_2)\geq a P(\phi_1)+(1-a)P(\phi_2).
\end{align}

If $\phi_1$ or $\phi_2$ makes the perturbed problem infeasible, then $P(\phi_1)=-\infty$ or $P(\phi_2)=-\infty$, and the inequality above is trivially true. Now, we just have to consider perturbations $\phi_1$ and $\phi_2$ that keep the perturbed problems feasible.

Let $d_{\rho}^{\pi_1}$/$d_{\rho}^{\pi_2}$ denote the discounted visitation distributions under initial distribution $\rho$ and policy $\pi_1$/$\pi_2$. For any $a\in[0,1]$, let us consider the policy $pi_a$ such that 
\begin{align*}
    d_{\rho}^{\pi_a}=a d_{\rho}^{\pi_1}+(1-a)d_{\rho}^{\pi_2}
\end{align*}
It is known that such a policy always exists. Note that the value function is linear in the discounted visitation distribution. As a result, we know
\begin{align}
    V_{i}^{\pi_a}=a V_{i}^{\pi_1}+(1-a)V_{i}^{\pi_2} \quad\forall i=0,1,\cdots,N.
\end{align}
Therefore,
\begin{align*}
    P(a\phi_1+(1-a)\phi_2)\geq V_{0}^{\pi_a}=V_{0}^{\pi_1}+(1-a)V_{0}^{\pi_2}=aP(\phi_1)+(1-a)P(\phi_2),
\end{align*}
which concludes the proof.

\qed



\subsection{Proof of Lemma \ref{lem:bounded_lambdastar}}
Let $\bar{\pi}$ denote the policy that satisfies the Slater's condition in Assumption \ref{assump:Slater}.
By the definition of the dual function,
\begin{align}
    V_D^{\lambda^{\star}}(\rho)\geq V_0^{\bar{\pi}}+(V_g^{\bar{\pi}}-b)^{\top}\lambda^{\star}\geq V_0^{\bar{\pi}}+\xi\sum_{i=1}^{N}\lambda_i^{\star}\geq V_0^{\bar{\pi}}+\xi\|\lambda^{\star}\|_{\infty}
\end{align}

Re-arranging the inequality and recognizing $V_D^{\lambda^{\star}}(\rho)=V_0^{\pi^{\star}}$ as implied by the strong duality in \eqref{lem:strong_duality} leads to
\begin{align}
    \|\lambda^\star\|_{\infty}\leq \frac{1}{\xi}(V_D^{\lambda^{\star}}(\rho)-V_0^{\bar{\pi}})=\frac{1}{\xi}(V_0^{\pi^{\star}}(\rho)-V_0^{\bar{\pi}}(\rho))\leq \frac{2}{\xi(1-\gamma)},
\end{align}
where the last inequality follows from bounded reward function (and hence bounded value function).

\qed



\subsection{Proof of Lemma \ref{lem:constraint_violation}}
Recall the perturbation function $P(\phi)$ defined in \eqref{eq:perturbation_def}. Then, we have for any $\pi$
\begin{align}
    V_{L}^{\pi,\lambda^{\star}}(\rho) \leq \max_{\pi} V_{L}^{\pi,\lambda^{\star}}(\rho)=V_{D}^{\lambda^{\star}}(\rho)=V_{0}^{\pi^{\star}}(\rho)=P(0),
    \label{lem:constraint_violation:eq1}
\end{align}
where the first equality uses the definition of the dual function, and the second equality comes from the strong duality.

Given $\phi \in \mathbb{R}^{N}$, we let $\pi_{\phi}$ denote that policy that attains the optimum for $P(\phi)$, i.e.
\begin{align*}
    \pi_{\phi}=\argmax V_0^{\pi}(\rho) \quad\text{subject to}\quad V_i^{\pi}(\rho)\geq b_i+\phi_i\quad\forall i=1,\cdots,N.
\end{align*}

Then, from \eqref{lem:constraint_violation:eq1} we have
\begin{align}
    P(0)-\langle\phi,\lambda^{\star}\rangle&\geq V_{L}^{\pi_{\phi},\lambda^{\star}}(\rho)-\langle\phi,\lambda^{\star}\rangle=V_{0}^{\pi_{\phi}}(\rho)+\langle\lambda^{\star},V_{g}^{\pi_{\phi}}(\rho)-b\rangle-\langle\phi,\lambda^{\star}\rangle\notag\\
    &=V_{0}^{\pi_{\phi}}(\rho)+\langle\lambda^{\star},V_{g}^{\pi_{\phi}}(\rho)-b-\phi\rangle=P(\phi).
\end{align}

Now, plugging $\phi=\bar{\phi}\triangleq-[b-V_g^{\bar{\pi}}(\rho)]_{+}$ into this result, we have
\begin{align}
    \langle\bar{\phi},\lambda^{\star}\rangle\leq P(0)- P(\bar{\phi}).
    \label{lem:constraint_violation:eq2}
\end{align}

Also, since $\bar{\phi}$ is non-positive,
\begin{align}
    V_0^{\bar{\pi}}(\rho)\leq V_0^{\pi^{\star}}(\rho)=P(0)\leq P(\bar{\phi}).
    \label{lem:constraint_violation:eq3}
\end{align}

Combining \eqref{lem:constraint_violation:eq2} and \eqref{lem:constraint_violation:eq3} implies
\begin{align}
    \langle\bar{\phi},\lambda^{\star}\rangle\leq P(0)-P(\bar{\phi}) \leq V_0^{\pi^{\star}}(\rho)-V_0^{\bar{\pi}}(\rho).
\end{align}
Then, since $\lambda^{\star}$ is entry-wise non-negative and $\bar{\phi}$ is entry-wise non-positive,
\begin{align}
    (C-\|\lambda^{\star}\|_{\infty})\|\bar{\phi}\|_{1} &\leq \langle \lambda^{\star}-C\1, \bar{\phi}\rangle \leq V_0^{\pi^{\star}}(\rho)-V_0^{\bar{\pi}}(\rho)+C\|\bar{\phi}\|_1 \notag\\
    &=V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\bar{\pi}}(\rho)+C\sum_{i=1}^{N}[b_i-V_i^{\bar{\pi}}(\rho)]_{+}\leq\delta.
\end{align}

Therefore,
\begin{align}
    \sum_{i=1}^{N}[b_i-V_i^{\bar{\pi}}(\rho)]_{+}=\|\bar{\phi}\|_{1}\leq \frac{\delta}{C-\|\lambda^{\star}\|_{\infty}}\leq \frac{2\delta}{C}.
\end{align}

\qed





\subsection{Proof of Lemma \ref{lem:bounded_Lagrangian}}
Again, from the performance difference lemma, 
\begin{align}
& V_{0}^{\pi^{\star}}(\rho)-V_0^{\pi_k}(\rho)\notag\\
&= \mathbb{E}_{s \sim \mu_{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[A_{0}^{\pi_k}(s, a)\right] \notag\\
&=\mathbb{E}_{s \sim \mu_{\pi^{\star}},a\sim\pi^{\star}(\cdot\mid s)}\left[ Q_{0}^{\pi_k}(s, a)\right]-\mathbb{E}_{s \sim \mu_{\pi^{\star}}}\left[V_{0}^{\pi_k}(s)\right]\notag\\
&=\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[\widehat{Q}_{L,k}(s, a)\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[\widehat{Q}_{g,k}(s, a)\right]\notag\\
&\hspace{20pt}+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[V_{0}^{\pi_k}(s)\right] \notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[\log\left(\frac{\pi_{k+1}(a\mid s)}{\pi_k(a\mid s)}\widehat{Z}_k\right)\right]\notag\\
&\hspace{20pt}-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[\widehat{A}_{g,k}(s, a)\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[\widehat{V}_{g,k}(s)\right]\notag\\
&\hspace{20pt}+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[V_{0}^{\pi_k}(s)\right] \notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
&\hspace{20pt}+\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[\log\widehat{Z}_k\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[\widehat{A}_{g,k}(s, a)\right]\notag\\
&\hspace{20pt}-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[\widehat{V}_{g,k}(s)\right]+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]\notag\\
&\hspace{20pt}-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[\widehat{V}_{0,k}(s)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi^{\star}}}\left[V_{0}^{\pi_k}(s)-\widehat{V}_{0,k}(s)\right].
\end{align}

Re-grouping the terms,
\begin{align}
& V_{0}^{\pi^{\star}}(\rho)-V_0^{\pi_k}(\rho)\notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
&\hspace{20pt}+\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\log\widehat{Z}_k\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[A_{g}^{\pi_k}(s, a)\right]\notag\\
&\hspace{20pt}+\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[A_{g}^{\pi_k}(s, a)-\widehat{A}_{g,k}(s, a)\right]\notag\\
&\hspace{20pt}-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\widehat{V}_{L,k}(s)\right]+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[A_{0}^{\pi_k}(s,a)-\widehat{A}_{0,k}(s, a)\right]\notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
&\hspace{20pt}+\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\log\widehat{Z}_k\right]-\lambda_k^{\top}\left(V_{g}^{\pi^{\star}}(\rho)-V_{g}^{\pi_k}(\rho)\right)\notag\\
&\hspace{20pt}-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\widehat{V}_{L,k}(s)\right]+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}, a \sim \pi^{\star}(\cdot \mid s)}\left[A_{L,k}^{\pi_k}(s, a)-\widehat{A}_{L,k}(s, a)\right]
% &\leq\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
% &\hspace{20pt}+\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\log\widehat{Z}_k\right]-\lambda_k^{\top}\left(V_{g}^{\pi^{\star}}(s)-V_{g}^{\pi_k}(s)\right)\notag\\
% &\hspace{20pt}-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\widehat{V}_{L,k}(s)\right]+\frac{1}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|
\label{lem:bounded_Lagrangian:eq1}
\end{align}

Using Lemma \ref{lem:step_improvement} with $\mu=d_{\rho}^{\pi^{\star}}$, we get
\begin{align}
    &\frac{1}{\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\log\widehat{Z}_k(s)\right]-\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[\widehat{V}_{L,k}(s)\right]\notag\\
    &\leq V_{0}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{0}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})+\lambda_k^{\top}\left(V_{g}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{g}^{\pi_k}(d_{\rho}^{\pi^{\star}})\right)+\frac{3-\gamma}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|.
    \label{lem:bounded_Lagrangian:eq2}
\end{align}


Combining \eqref{lem:bounded_Lagrangian:eq1} and \eqref{lem:bounded_Lagrangian:eq2}, we have
\begin{align}
    % &V_{0}^{\pi^{\star}}(\rho)-V_0^{\pi_k}(\rho)+\lambda_k^{\top}\left(V_{g}^{\pi^{\star}}(\rho)-V_g^{\pi_k}(\rho)\right)\notag\\
    &V_{L,k}^{\pi^{\star}}(\rho)-V_{L,k}^{\pi_{k}}(\rho)\notag\\
    &\leq \frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\left(V_{0}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{0}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})+\lambda_k^{\top}\left(V_{g}^{\pi_{k+1}}(s)-V_{g}^{\pi_k}(s)\right)+\frac{3-\gamma}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\right)\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\notag\\
    &\leq \frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))\right]-\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{KL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\left(V_{L,k}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{L,k}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{4-2\gamma}{(1-\gamma)^2}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|
\end{align}

(Use fixed step sizes $\alpha_k=\alpha$, $\eta_k=\eta$)


Taking the sum from $k=0$ to $k=K-1$,
\begin{align}
    \frac{1}{K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi^{\star}}(\rho)-V_{L,k}^{\pi_{k}}(\rho)\right) &\leq \frac{1}{(1-\gamma)K\alpha}\sum_{k=0}^{K-1}\mathbb{E}_{s\sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{DL}}(\pi^{\star}(\cdot\mid s)||\pi_k(\cdot\mid s))-D_{\text{DL}}(\pi^{\star}(\cdot\mid s)||\pi_{k+1}(\cdot\mid s))\right]\notag\\
    &\hspace{20pt}+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{L,k}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\notag\\
    &\leq \frac{1}{(1-\gamma)K\alpha}\mathbb{E}_{s\sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{DL}}(\pi^{\star}(\cdot\mid s)||\pi_0(\cdot\mid s))\right]\notag\\
    &\hspace{20pt}+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{L,k}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|.
    \label{lem:bounded_Lagrangian:eq3}
\end{align}

The second term on the RHS can be treated as follows
\begin{align}
    &\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{L,k}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)\notag\\
    &\leq \frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{0}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\lambda_k^{\top}\left(V_{0}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{0}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)\notag\\
    &= \frac{V_{0}^{\pi_{K}}(d_{\rho}^{\pi^{\star}})}{(1-\gamma)K}+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(\lambda_{k+1}^{\top}V_{g}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-\lambda_k^{\top}V_{g}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(\lambda_{k}^{\top}-\lambda_{k+1}^{\top}\right)V_{g}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})\notag\\
    &= \frac{V_{0}^{\pi_{K}}(d_{\rho}^{\pi^{\star}})}{(1-\gamma)K}+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(\lambda_{k+1}^{\top}V_{g}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-\lambda_k^{\top}V_{g}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(\lambda_{k}^{\top}-\lambda_{k+1}^{\top}\right)V_{g}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})\notag\\
    &= \frac{V_{0}^{\pi_{K}}(d_{\rho}^{\pi^{\star}})}{(1-\gamma)K}+\frac{1}{(1-\gamma) K}\sum_{i=1}^{N}\lambda_{i,K}V_i^{\pi_K}(d_{\rho}^{\pi^{\star}})+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}(\lambda_{i,k}-\lambda_{i,k+1})V_{i}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}}).
    \label{lem:bounded_Lagrangian:eq4}
\end{align}

Due to the bounded reward functions, we know that $V_{i}^{\pi}(\mu)\leq\frac{1}{1-\gamma}$ for all $\pi$, $\mu$, and $i=1,2,\cdots,N$. Also the dual variable update \eqref{Alg:AC:dual_update} implies \eqref{eq:lambda_ik_bound}. Using the bounds on the value functions and $|\lambda_{i,k}|$ in \eqref{lem:bounded_Lagrangian:eq4}, we have
\begin{align*}
    &\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})-V_{L,k}^{\pi_{k}}(d_{\rho}^{\pi^{\star}})\right)\notag\\
    &\leq \frac{V_{0}^{\pi_{K}}(d_{\rho}^{\pi^{\star}})}{(1-\gamma)K}+\frac{1}{(1-\gamma) K}\sum_{i=1}^{N}\lambda_{i,K}V_i^{\pi_K}(d_{\rho}^{\pi^{\star}})+\frac{1}{(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}(\lambda_{i,k}-\lambda_{i,k+1})V_{i}^{\pi_{k+1}}(d_{\rho}^{\pi^{\star}})\notag\\
    &\leq \frac{1}{(1-\gamma)^2 K}+\frac{2N}{\xi(1-\gamma)^3 K}+\frac{2N}{\xi(1-\gamma)^3 K} \leq\frac{6N}{\xi(1-\gamma)^3 K}.
\end{align*}

Combining this with \eqref{lem:bounded_Lagrangian:eq3} implies
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{L,k}^{\pi^{\star}}(\rho)-V_{L,k}^{\pi_{k}}(\rho)\right)\notag\\
    &\leq \frac{1}{(1-\gamma)K\alpha}\mathbb{E}_{s\sim d_{\rho}^{\pi^{\star}}}\left[D_{\text{DL}}(\pi^{\star}(\cdot\mid s)||\pi_0(\cdot\mid s))\right]+\frac{6N\eta}{(1-\gamma)^3}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|,
\end{align}
where the last inequality uses the fact that for $D_{\text{KL}}(p_1||p_2)\leq\log|\Acal|$ for $p_1,p_2\in\Delta_{\Acal}$ if $p_2$ is a uniform distribution.

\qed





\subsection{Proof of Lemma \ref{lem:step_improvement}}
\begin{align*}
V_{0}^{\pi_{k+1}}(\mu)-V_{0}^{\pi_{k}}(\mu)&= \frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[A_{0}^{\pi_k}(s, a)\right] \notag\\
&= \frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s, a)\right] -\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[V_{0}^{\pi_k}(s)\right] \notag\\
&=\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[\widehat{Q}_{L,k}(s, a)\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[\widehat{Q}_{g,k}(s, a)\right]\notag\\
&\hspace{20pt}+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[V_{0}^{\pi_k}(s)\right] \notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[\log\left(\frac{\pi_{k+1}(a\mid s)}{\pi_k(a\mid s)}\widehat{Z}_k(s)\right)\right]\notag\\
&\hspace{20pt}-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[\widehat{A}_{g,k}(s, a)\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{g,k}(s)\right]\notag\\
&\hspace{20pt}+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[V_{0}^{\pi_k}(s)\right] \notag\\
&=\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[D_{\text{KL}}(\pi_{k+1}(\cdot\mid s)||\pi_{k}(\cdot\mid s))\right]+\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\log\widehat{Z}_k(s)\right]\notag\\
&\hspace{20pt}-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[\widehat{A}_{g,k}(s, a)\right]-\frac{\lambda_k^{\top}}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{g,k}(s)\right]\notag\\
&\hspace{20pt}+\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}, a \sim \pi_{k+1}(\cdot \mid s)}\left[Q_{0}^{\pi_k}(s,a)-\widehat{Q}_{0,k}(s, a)\right]-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{0,k}(s)\right]\notag\\
&\hspace{20pt}-\frac{1}{1-\gamma}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[V_{0}^{\pi_k}(s)-\widehat{V}_{0,k}(s)\right] \notag\\
&\geq \frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\log\widehat{Z}_k(s)\right]-\frac{1}{(1-\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{L,k}(s)\right]\notag\\
&\hspace{20pt}-\frac{\lambda_k^{\top}}{(1\hspace{-2pt}-\hspace{-2pt}\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}\hspace{-3pt},a\sim\pi_{k+1}(\cdot\mid s)}\hspace{-2pt}\left[\hspace{-1pt}A_{g}^{\pi_k}(s)\hspace{-1pt}\right]\hspace{-2pt}+\hspace{-2pt}\frac{1}{(1\hspace{-2pt}-\hspace{-2pt}\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}\hspace{-3pt},a\sim\pi_{k+1}(\cdot\mid s)}\hspace{-2pt}\left[\hspace{-2pt}A_{L,k}^{\pi_k}(s,a)\hspace{-2pt}-\hspace{-2pt}\widehat{A}_{L,k}(s,a)\right].
\end{align*}

Re-arranging the inequality and using the performance difference,
\begin{align}
&V_{0}^{\pi_{k+1}}(\mu)-V_{0}^{\pi_{k}}(\mu)+\lambda_k^{\top}\left(V_{g}^{\pi_{k+1}}(\mu)-V_{g}^{\pi_k}(\mu)\right)\notag\\ &\geq\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\log\widehat{Z}_k(s)\right]-\frac{1}{(1-\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{L,k}(s)\right]\notag\\
&\hspace{20pt}+\frac{1}{(1-\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}},a\sim\pi_{k+1}(\cdot\mid s)}\left[A_{L,k}^{\pi_k}(s,a)-\widehat{A}_{L,k}(s,a)\right]\notag\\
&\geq\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\log\widehat{Z}_k(s)\right]-\frac{1}{(1-\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{L,k}(s)\right]-\frac{1}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|.
\label{lem:step_improvement:eq1}
\end{align}


We can show that
\begin{align}
    \log\widehat{Z}_k(s)&=\log \left(\sum_{a'\in\Acal}\pi_k(a' \mid s) \exp \left(\alpha_k \widehat{Q}_{L,k}(s, a')\right)\right)\notag\\
    &\geq \sum_{a'\in\Acal}\pi_k(a' \mid s)\log \left( \exp \left(\alpha_k \widehat{Q}_{L,k}(s, a')\right)\right)\notag\\
    &= \alpha_k \sum_{a'\in\Acal}\pi_k(a' \mid s_k)\widehat{Q}_{L,k}(s, a')\notag\\
    &= \alpha_k\widehat{V}_{L,k}(s) + \alpha_k \sum_{a'\in\Acal}\pi_k(a' \mid s_k)\widehat{A}_{L,k}(s, a')\notag\\
    &= \alpha_k\widehat{V}_{L,k}(s) + \alpha_k \sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right),
\end{align}
where the last inequality uses the fact that $\sum_{a'\in\Acal}\pi_k(a' \mid s_k)A_{L,k}^{\pi_k}(s,a')=0$. 

This inequality implies that 
\begin{align}
    &\frac{1}{(1-\gamma)\alpha_k}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\log\widehat{Z}_k(s)\right]-\frac{1}{(1-\gamma)}\mathbb{E}_{s \sim d_{\mu}^{\pi_{k+1}}}\left[\widehat{V}_{L,k}(s)\right]\notag\\
    &=\frac{1}{(1-\gamma)\alpha_k}\sum_{s\in\Scal}d_{\mu}^{\pi_{k+1}}(s)\left(\log\widehat{Z}_k(s)-\alpha_k \widehat{V}_{L,k}(s)-\alpha_k\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\right)\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\sum_{s\in\Scal}d_{\mu}^{\pi_{k+1}}(s)\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\notag\\
    &\geq \frac{1}{\alpha_k}\sum_{s\in\Scal}\mu(s)\left(\log\widehat{Z}_k(s)-\alpha_k \widehat{V}_{L,k}(s)-\alpha_k\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\right)\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\sum_{s\in\Scal}d_{\mu}^{\pi_{k+1}}(s)\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\notag\\
    &\geq \frac{1}{\alpha_k}\mathbb{E}_{s \sim \mu}\left[\log\widehat{Z}_k(s)\right]-\mathbb{E}_{s \sim \mu}\left[\widehat{V}_{L,k}(s)\right]-\sum_{s\in\Scal}\mu(s)\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\notag\\
    &\hspace{20pt}+\frac{1}{1-\gamma}\sum_{s\in\Scal}d_{\mu}^{\pi_{k+1}}(s)\sum_{a'\in\Acal}\pi_k(a' \mid s_k)\left(\widehat{A}_{L,k}(s, a')-A_{L,k}^{\pi_k}(s,a')\right)\notag\\
    &\geq \frac{1}{\alpha_k}\mathbb{E}_{s \sim \mu}\left[\log\widehat{Z}_k(s)\right]-\mathbb{E}_{s \sim \mu}\left[\widehat{V}_{L,k}(s)\right]-\frac{2-\gamma}{1-\gamma}\|\widehat{A}_{L,k}-A_{L,k}^{\pi_k}\|,
\end{align}
where the first inequality uses $d_{\mu}^{(t+1)} \geq(1-\gamma) \mu$ elementwise.

Combining this inequality with \eqref{lem:step_improvement:eq1} yields
\begin{align*}
    V_{0}^{\pi_{k+1}}(\mu)-V_{0}^{\pi_{k}}(\mu)+\lambda_k^{\top}\left(V_{g}^{\pi_{k+1}}(\mu)-V_{g}^{\pi_k}(\mu)\right)\geq\frac{1}{\alpha_k}\mathbb{E}_{s \sim \mu}\left[\log\widehat{Z}_k(s)\right]-\mathbb{E}_{s \sim \mu}\left[\widehat{V}_{L,k}(s)\right]-\frac{3-\gamma}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|.
\end{align*}

\qed


==> OldFiles/Oct19_Proofs/Proof_Notations.tex <==
\section{Proof of Main Results}


We introduce a few shorthand notations that will be used in the rest of the paper. First, we define $\widehat{V}_{i,k}\in\mathbb{R}^{|\Scal|}$ and $\widehat{A}_{i,k}\in\mathbb{R}^{|\Scal|\times|\Acal|}$ such that
\begin{align*}
    \widehat{V}_{i,k}(s)=\sum_{a'\in\Acal}\pi_k(a'\mid s)\widehat{Q}_{i,k}(s,a'),\quad\text{and}\quad \widehat{A}_{i,k}(s,a) = \widehat{Q}_{i,k}(s,a)-\widehat{V}_{i,k}(s),\quad\forall s\in\Scal,a\in\Acal.
\end{align*}


We use the subscript $g$ under a value/Q/advantage function to denote the vector formed by stacking the value/Q/advantage functions over the utilities, i.e.
\begin{align*}
    &V_{g}^{\pi}(s) \triangleq [V_{1}^{\pi}(s),...,V_{N}^{\pi}(s)]^{\top}\in\mathbb{R}^{N}\\
    &\widehat{V}_{g,k}(s) \triangleq [\widehat{V}_{1,k}(s),...,\widehat{V}_{N,k}(s)]^{\top}\in\mathbb{R}^{N}\\
    &Q_{g}^{\pi}(s,a) \triangleq [Q_{1}^{\pi}(s,a),...,Q_{N}^{\pi}(s,a)]^{\top}\in\mathbb{R}^{N}\\
    &\widehat{Q}_{g,k}(s,a) \triangleq [\widehat{Q}_{1,k}(s,a),...,\widehat{Q}_{N,k}(s,a)]^{\top}\in\mathbb{R}^{N}\\
    &A_{g}^{\pi}(s,a) \triangleq [A_{1}^{\pi}(s,a),...,A_{N}^{\pi}(s,a)]^{\top}\in\mathbb{R}^{N}\\
    &\widehat{A}_{g,k}(s,a) \triangleq [\widehat{A}_{1,k}(s,a),...,\widehat{A}_{N,k}(s,a)]^{\top}\in\mathbb{R}^{N}.
\end{align*}
The subscript $L,k$ denotes the sum over reward and utilities of the value/Q/advantage functions, weighted by the dual variable in the $k$-th iteration, i.e.
\begin{align*}
    &V_{L,k}(s)\triangleq V_{0}^{\pi_k}(s)+\lambda_k^{\top} V_{g}^{\pi_k}(s)\in\mathbb{R}\\
    &\widehat{V}_{L,k}(s)\triangleq \widehat{V}_{0,k}(s)+\lambda_k^{\top} \widehat{V}_{g,k}(s)\in\mathbb{R}\\
    &Q_{L,k}(s, a)\triangleq Q_{0}^{\pi_k}(s, a)+\lambda_k^{\top} Q_{g}^{\pi_k}(s, a)\in\mathbb{R}\\
    &\widehat{Q}_{L,k}(s, a)\triangleq \widehat{Q}_{0,k}(s, a)+\lambda_k^{\top} \widehat{Q}_{g,k}(s, a)\in\mathbb{R}\\
    &A_{L,k}(s, a)\triangleq A_{0}^{\pi_k}(s, a)+\lambda_k^{\top} A_{g}^{\pi_k}(s, a)\in\mathbb{R}\\
    &\widehat{A}_{L,k}(s, a)\triangleq \widehat{A}_{0,k}(s, a)+\lambda_k^{\top} \widehat{A}_{g,k}(s, a)\in\mathbb{R}.
\end{align*}



There is a simple bound we will frequently use that follows the boundedness of the reward and utility functions
\begin{align}
    % &|\lambda_{i,k}|\leq \frac{2}{\xi(1-\gamma)},\,\text{and }
    |\lambda_{i,k}-\lambda_{i,k+1}|\leq \frac{2\eta}{1-\gamma},\,\forall i=1,2,\cdot,N, \,\,k=0,1,\cdots,K-1.\label{eq:lambda_ik_bound}
\end{align}

We define the perturbation function for $\phi\in\mathbb{R}^{N}$
\begin{align}
    P(\phi)\triangleq \max_{\pi}&\quad V_0^{\pi}(\rho)\notag\\
    \text{subject to }&\quad V_i^{\pi}(\rho)\geq b_i+\phi_i\quad\forall i=1,\cdots,N,
    \label{eq:perturbation_def}
\end{align}
which plays an important role in establishing the strong duality for the problem \eqref{eq:Lagrangian}.

We also introduce the following technical lemmas.


\begin{lem}\label{lem:perturbation_concave}
The perturbation function defined in \eqref{eq:perturbation_def} is concave.
\end{lem}



\begin{lem}\label{lem:constraint_violation}
Under Assumption \ref{assump:Slater}, for any $C\geq 2\|\lambda^{\star}\|_{\infty}$, if there exists a policy $\bar{\pi}\in\Delta_{\Acal}^{\Scal}$ and $\delta>0$ such that
\begin{align*}
    V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\bar{\pi}}(\rho)+C\sum_{i=1}^{N}[b_i-V_i^{\bar{\pi}}(\rho)]_{+}\leq\delta,
\end{align*}
then we have
\begin{align*}
    \sum_{i=1}^{N}[b_i-V_i^{\bar{\pi}}(\rho)]_{+}\leq \frac{2\delta}{C}.
\end{align*}
\end{lem}




\begin{lem}\label{lem:bounded_Lagrangian}
Bounded Lagrangian
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)+\lambda_k^{\top}\left(V_{g}^{\pi^{\star}}(\rho)-V_{g}^{\pi_{k}}(\rho)\right)\right)\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|
\end{align}
\end{lem}





==> OldFiles/Oct19_Proofs/Proof_Proposition.tex <==
\subsection{Proof of Proposition \ref{prop:convergence_obj_constraintviolation}}

We introduce an additional lemma that bounds the (approximate) Lagrangian averaged over iterations.


\begin{lem}\label{lem:step_improvement}
Improvement in objective function every step:
\begin{align*}
    &V_{0}^{\pi_{k+1}}(\mu)-V_{0}^{\pi_{k}}(\mu)+\lambda_k^{\top}\left(V_{g}^{\pi_{k+1}}(s)-V_{g}^{\pi_k}(s)\right)\notag\\
    &\geq\frac{1}{\alpha_k}\mathbb{E}_{s \sim \mu}\left[\log\widehat{Z}_k(s)\right]-\mathbb{E}_{s \sim \mu}\left[\widehat{V}_{L,k}(s)\right]-\frac{3-\gamma}{1-\gamma}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|
\end{align*}
for any initial distribution $\mu$.
\end{lem}



\noindent\textbf{Objective function convergence}
From the dual update \eqref{Alg:AC:dual_update}, we have
\begin{align}
    0\leq\|\lambda_K\|^2&=\sum_{k=0}^{K-1}\left(\|\lambda_{k+1}\|^2-\|\lambda_k\|^2\right)\notag\\
    &=\sum_{k=0}^{K-1}\left(\left\|\Pi\left(\lambda_k-\eta_k\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right)\right)\right\|^2-\|\lambda_k\|^2\right)\notag\\
    &\leq\sum_{k=0}^{K-1}\left(\left\|\lambda_k-\eta_k\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right)\right\|^2-\|\lambda_k\|^2\right)\notag\\
    &=-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right)+\eta^2\sum_{k=0}^{K-1}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right\|^2\notag\\
    &=-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)Q_{g}^{\pi_k}(s,a)-b\right)-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)(\widehat{Q}_{g,k}(s,a)-Q_{g}^{\pi_k}(s,a)\right)\notag\\
    &\hspace{20pt}+\eta^2\sum_{k=0}^{K-1}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right\|^2\notag\\
    &=-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(V_g^{\pi_k}(\rho)-b\right)-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)(\widehat{Q}_{g,k}(s,a)-Q_{g}^{\pi_k}(s,a)\right)\notag\\
    &\hspace{20pt}+\eta^2\sum_{k=0}^{K-1}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right\|^2,
    \label{prop:convergence_obj_constraintviolation:eq0}
\end{align}
where the first inequality follows from the fact that the projection operator is non-expansive, and the second inequality comes from the boundedness of the reward functions and the fact that $V_i^{\pi^{\star}}(\rho)\geq b_i$ for all $i=1,2,\cdots,N$.
By the Cauchy-Schwarz inequality the second term above can be bounded as
\begin{align}
    -\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)(\widehat{Q}_{g,k}(s,a)-Q_{g}^{\pi_k}(s,a)\right)&=-\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)(\widehat{Q}_{i,k}(s,a)-Q_{i}^{\pi_k}(s,a)\right)\notag\\
    &\leq \sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left(\sum_{s,a}\rho(s)^2\pi_k(a\mid s)^2\right)^{1/2}\|\widehat{Q}_{g,k}-Q_{g}^{\pi_k}\|\notag\\
    &\leq\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)\right)\|\widehat{Q}_{g,k}-Q_{g}^{\pi_k}\|\notag\\
    &\leq\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\|\widehat{Q}_{g,k}-Q_{g}^{\pi_k}\|.
    \label{prop:convergence_obj_constraintviolation:eq0.25}
\end{align}
In addition, the third term of \eqref{prop:convergence_obj_constraintviolation:eq0} follows from the fact that the value function and constant $b_i$ are all within $[0,\frac{1}{1-\gamma}]$.
\begin{align}
    \sum_{k=0}^{K-1}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right\|^2&= \sum_{k=0}^{K-1}\sum_{i=1}^{N}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{i,k}(s,a)-b_i\right\|^2\notag\\
    &\leq 2\sum_{k=0}^{K-1}\sum_{i=1}^{N}\left(\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{i,k}(s,a)\right\|^2+\left\|b_i\right\|^2\right)\notag\\
    &\leq 2\sum_{k=0}^{K-1}\sum_{i=1}^{N}\left(\frac{1}{(1-\gamma)^2}+\frac{1}{(1-\gamma)^2}\right)=\frac{4KN}{(1-\gamma)^2}.\label{prop:convergence_obj_constraintviolation:eq0.5}
\end{align}

Using \eqref{prop:convergence_obj_constraintviolation:eq0.25} and \eqref{prop:convergence_obj_constraintviolation:eq0.5} in \eqref{prop:convergence_obj_constraintviolation:eq0}, we get
\begin{align*}
    0&\leq-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(V_{g}^{\pi_k}(\rho)-b\right)-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(\sum_{s,a}\rho(s)\pi_k(a\mid s)(\widehat{Q}_{g,k}(s,a)-Q_{g}^{\pi_k}(s,a)\right)\notag\\
    &\hspace{20pt}+\eta^2\sum_{k=0}^{K-1}\left\|\sum_{s,a}\rho(s)\pi_k(a\mid s)\widehat{Q}_{g,k}(s,a)-b\right\|^2\notag\\
    &\leq-2\eta\sum_{k=0}^{K-1}\lambda_k^{\top}\left(V_{g}^{\pi_k}(\rho)-b\right)+2\eta\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|+\frac{4KN\eta^2}{(1-\gamma)^2}\notag\\
    &\leq 2\eta\sum_{k=0}^{K-1}\lambda_k^{\top} \left(V_{g}^{\pi^{\star}}(\rho)-V_{g}^{\pi_k}(\rho)\right)+2\eta\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|+\frac{4KN\eta^2}{(1-\gamma)^2},
\end{align*}
where the last inequality follows from the fact that the optimal policy satisfies the constraints, i.e. $V_i^{\pi^{\star}}(\rho)\geq b_i$ for all $i=1,\cdots,N$.

Re-arranging this inequality leads to
\begin{align}
    \frac{1}{K}\sum_{k=0}^{K-1}\lambda_k^{\top} \left(V_{g}^{\pi^{\star}}(\rho)-V_{g}^{\pi_k}(\rho)\right)\geq -\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\| - \frac{2N\eta}{(1-\gamma)^2}.
\end{align}


Combining this with Lemma \ref{lem:bounded_Lagrangian}, we get
\begin{align}
    \frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)\right)
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\notag\\
    &\hspace{20pt}+\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\lambda_{i,k}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\| + \frac{2N\eta}{(1-\gamma)^2}\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{4(2-\gamma)}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|\widehat{Q}_{0,k}-Q_{0}^{\pi_k}\|\notag\\
    &\hspace{20pt}+\left(\frac{8(2-\gamma)}{\xi(1-\gamma)^3 K }+\frac{2}{\xi(1-\gamma)K}\right)\sum_{k=0}^{K-1}\sum_{i=1}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\| + \frac{2N\eta}{(1-\gamma)^2}
    \label{prop:convergence_obj_constraintviolation:eq1}
\end{align}
where the last inequality follows from \eqref{eq:lambda_ik_bound} and
\begin{align}
    \sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|&\leq \sum_{k=0}^{K-1}\left(\|A_{0}^{\pi_k}-\widehat{A}_{0,k}\|+\sum_{i=1}^{N}|\lambda_{i,k}|\|A_{i}^{\pi_k}-\widehat{A}_{i,k}\|\right)\notag\\
    &\leq \sum_{k=0}^{K-1}\|A_{0}^{\pi_k}-\widehat{A}_{0,k}\|+\frac{2}{\xi(1-\gamma)}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|A_{i}^{\pi_k}-\widehat{A}_{i,k}\|\notag\\
    &\leq 2\sum_{k=0}^{K-1}\|Q_{0}^{\pi_k}-\widehat{Q}_{0,k}\|+\frac{4}{\xi(1-\gamma)}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|Q_{i}^{\pi_k}-\widehat{Q}_{i,k}\|.
    \label{eq:Q_bound_A}
\end{align}

% \sihan{need to check this}


Defining $C_1=\frac{8(2-\gamma)}{\xi(1-\gamma)^3}+\frac{4}{\xi(1-\gamma)}$ and combining terms in \eqref{prop:convergence_obj_constraintviolation:eq1}, we have
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)\right)
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+ \frac{2N\eta}{(1-\gamma)^2}+\frac{C_1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\| 
\end{align*}


\textbf{Constraint violation convergence}

For any $\lambda\in[0,\frac{2}{(1-\gamma)\xi}]^{N}$, since the projection operator is non-expansive, we have
\begin{align*}
    \|\lambda_{k+1}-\lambda\|^2 &= \|\Pi_{\mathbb{R}_{+}}(\lambda_k-\eta(\hat{V}_{g,k}(\rho)-b))-\lambda\|^2\notag\\
    &\leq \|\lambda_k-\eta(\hat{V}_{g,k}(\rho)-b)-\lambda\|^2\notag\\
    &= \|\lambda_k-\lambda\|^2-2\eta(\lambda_k-\lambda)^{\top}(\hat{V}_{g,k}(\rho)-b)+\eta^2\|\hat{V}_{g,k}(\rho)-b\|^2\notag\\
    &\leq \|\lambda_k-\lambda\|^2-2\eta(\lambda_k-\lambda)^{\top}(\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho))-2\eta(\lambda_k-\lambda)^{\top}(V_{g}^{\pi_k}(\rho)-b)+\frac{4N\eta^2}{(1-\gamma)^2}.
\end{align*}


Re-arranging the terms and summing up from $k=0$ to $K-1$, we get
\begin{align}
    &\frac{2\eta}{K}\sum_{k=0}^{K-1}(\lambda_k-\lambda)^{\top}(V_{g}^{\pi_k}(\rho)-b)\notag\\
    &\leq\frac{1}{K}\left(\|\lambda_0-\lambda\|^2-\|\lambda_K-\lambda\|^2\right)-\frac{2\eta}{K}\sum_{k=0}^{K-1}(\lambda_k-\lambda)^{\top}(\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho))+\frac{4N\eta^2}{(1-\gamma)^2}\notag\\
    &\leq \frac{1}{K}\|\lambda_0-\lambda\|^2+\frac{2\eta}{K}\sum_{k=0}^{K-1}\|\lambda_k-\lambda\|\|\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho)\|+\frac{4N\eta^2}{(1-\gamma)^2}
    \label{eq:constraint_violation_1}
\end{align}


To bound the second term of this inequality, we consider
\begin{align}
    \frac{2\eta}{K}\sum_{k=0}^{K-1}\|\lambda_k-\lambda\|\|\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho)\|&\leq \frac{2\eta}{K}\sum_{k=0}^{K-1}\left(\|\lambda_k\|+\|\lambda\|\right)\|\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho)\|\notag\\
    &\leq \frac{2\eta}{K}\sum_{k=0}^{K-1}\left(\frac{2}{\xi(1-\gamma)}+\frac{2}{\xi(1-\gamma)}\right)\|\hat{V}_{g,k}(\rho)-V_{g}^{\pi_k}(\rho)\|\notag\\
    &\leq \frac{8\eta}{\xi(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|
    \label{eq:constraint_violation_2}
\end{align}

Using \eqref{eq:constraint_violation_2} in \eqref{eq:constraint_violation_1} and dividing both sides by $2\eta$, we get
\begin{align}
    \frac{1}{K}\sum_{k=0}^{K-1}(\lambda_k-\lambda)^{\top}(V_{g}^{\pi_k}(\rho)-b) &\leq \frac{1}{2K\eta}\|\lambda_0-\lambda\|^2+\frac{4}{\xi(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|
    +\frac{2N\eta}{(1-\gamma)^2}
    \label{eq:constraint_violation_3}
\end{align}




Adding \eqref{eq:constraint_violation_3} to the result of Lemma \ref{lem:bounded_Lagrangian}, we have
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)+\lambda_k^{\top}\left(V_{g}^{\pi^{\star}}(\rho)-b\right)+\lambda^{\top}(V_g^{\pi_k}(\rho)-b)\right)\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|\notag\\
    &\hspace{20pt}+\frac{1}{2K\eta}\|\lambda_0-\lambda\|^2+\frac{4}{\xi(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|
    +\frac{2N\eta}{(1-\gamma)^2}
\end{align}
Combining the terms and using the fact that $V_g^{\pi_k}(\rho)-b\geq 0$, this inequality implies
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)+\lambda^{\top}(b-V_g^{\pi_k}(\rho))\right)\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{1}{2K\eta}\|\lambda_0-\lambda\|^2\notag\\
    &\hspace{20pt}+\frac{4-2\gamma}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|A_{L,k}^{\pi_k}-\widehat{A}_{L,k}\|+\frac{4}{\xi(1-\gamma)K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{1}{2K\eta}\|\lambda_0-\lambda\|^2\notag\\
    &\hspace{20pt}+\frac{4(2-\gamma)}{(1-\gamma)^2 K}\sum_{k=0}^{K-1}\|Q_{0}^{\pi_k}-\widehat{Q}_{0,k}\|+\left(\frac{8(2-\gamma)}{\xi(1-\gamma)^3 K}+\frac{4}{\xi(1-\gamma)K}\right)\sum_{k=0}^{K-1}\sum_{i=1}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|\notag\\
    &= \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{1}{2K\eta}\|\lambda_0-\lambda\|^2+\frac{C_1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|,
    \label{eq:constraint_violation_4}
\end{align}
where the second inequality again follows from \eqref{eq:Q_bound_A}, and the equality uses the constant definition $C_1=\frac{8(2-\gamma)}{\xi(1-\gamma)^3}+\frac{4}{\xi(1-\gamma)}$.


Now, choosing $\lambda$ such that 
\begin{align*}
    \lambda_i = \begin{cases}\frac{4}{(1-\gamma)\xi}, & \text { if } b_i-V_i^{\pi_k}(\rho)\geq 0 \\ 0, & \text { else }\end{cases}
\end{align*}
Then, \eqref{eq:constraint_violation_4} leads to
\begin{align}
    &\frac{1}{K}\sum_{k=0}^{K-1}\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\pi_{k}}(\rho)\right)+\frac{1}{K}\sum_{k=0}^{K-1}\sum_{i=1}^{N}\frac{4}{(1-\gamma)\xi}\Big[b_i-V_{i}^{\pi_k}(\rho)\Big]_{+}\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{1}{2K\eta}\cdot\frac{16N}{\xi^2(1-\gamma)^2}+\frac{C_1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|
    \label{eq:constraint_violation_5}
\end{align}

Note that there always exists a policy $\bar{\pi}_K$ such that $d_{\rho}^{\bar{\pi}_K}=\frac{1}{K}\sum_{k=0}^{K-1}d_{\rho}^{\pi_k}$, which implies
\begin{align*}
    V_i^{\bar{\pi}_K}=\frac{1}{K}\sum_{k=0}^{K-1} V_i^{\pi_k}\quad\forall i=0,1,\cdots,N.
\end{align*}

As a result, \eqref{eq:constraint_violation_5} becomes
\begin{align}
    &\left(V_{0}^{\pi^{\star}}(\rho)-V_{0}^{\bar{\pi}_{K}}(\rho)\right)+\frac{4}{(1-\gamma)\xi}\sum_{i=1}^{N}\Big[b_i-V_{i}^{\bar{\pi}_{K}}(\rho)\Big]_{+}\notag\\
    &\leq \frac{\log|\Acal|}{(1-\gamma)K\alpha}+\frac{6N}{\xi(1-\gamma)^3 K}+\frac{2N\eta}{(1-\gamma)^2}+\frac{8N}{K\eta\xi^2(1-\gamma)^2}+\frac{C_1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\left\|\widehat{Q}_{i,k}-Q_{i}^{\pi_k}\right\|
\end{align}


Recall that Lemma \ref{lem:bounded_lambdastar} states that $2\|\lambda^{\star}\|_{\infty}\leq\frac{4}{(1-\gamma)\xi}$. Applying Lemma \ref{lem:constraint_violation} with $C=\frac{4}{(1-\gamma)\xi}$, we have
\begin{align*}
    \sum_{i=1}^{N}\Big[b_i-V_{i}^{\bar{\pi}_{K}}(\rho)\Big]_{+}\hspace{-2pt}&\leq\hspace{-2pt}\frac{\xi(1-\gamma)}{2}\Big(\frac{\log|\Acal|}{(1-\gamma)K\alpha}\hspace{-2pt}+\hspace{-2pt}\frac{6N}{\xi(1-\gamma)^3 K}\hspace{-2pt}+\hspace{-2pt}\frac{2N\eta}{(1-\gamma)^2}\hspace{-2pt}+\hspace{-2pt}\frac{8N}{K\eta\xi^2(1-\gamma)^2}\hspace{-2pt}+\hspace{-2pt}\frac{C_1}{K}\sum_{k=0}^{K-1}\sum_{i=0}^{N}\|\hat{Q}_{i,k}-Q_{i}^{\pi_k}\|\Big).
\end{align*}

\qed





\subsection{Proof of Proposition \ref{prop:conv_critic}}

We define some convenient shorthand notations used in the proof of Proposition \ref{prop:conv_critic}.
\begin{align*}
    &O_k=(s_k,a_k,s_{k+1},a_{k+1})\notag\\
    &R_i(O_k)\in\mathbb{R}^{|\Scal||\Acal|}\text{  where  } R_i(O_k)_m= \begin{cases} r_i(s_k,a_k), & \text { if } m=(s_k,a_k) \\ 0, &\text{ otherwise}\end{cases}\\
    &M(O)=M(s,a,s',a')\in\mathbb{R}^{|\Scal||\Acal|\times |\Scal||\Acal|}\text{  where if } (s,a=s',a'): \begin{aligned}
    M(O)_{m,n}=\begin{cases} \gamma-1, & \text{if } m=n=(s,a) \\ 0, & \text { otherwise}\end{cases}\end{aligned}\\
    &\hspace{194pt}\text{if }(s,a\neq s',a'): \begin{aligned} M(O)_{m,n}=\begin{cases} -1, & \text { if } m=n=(s,a) \\
    \gamma, & \text { if, } m=(s,a),n=(s',a') \\ 
    0, & \text { otherwise}\end{cases}
    \end{aligned}
\end{align*}

For any policy $\pi$, we define
\begin{align*}
    &\widebar{M}^{\pi}=\mathbb{E}_{s\sim\mu_{\pi},a\sim\pi(\cdot\mid s),s'\sim\Pcal(\cdot\mid s,a),a'\sim\pi(\cdot\mid s')}[M(s,a,s',a')],\\
    &\Gamma_i(\pi,z,O)=z^{\top}(R_i(O)+M(O)Q_i^{\pi})+z^{\top}(M(O)-\widebar{M}^{\pi})z
\end{align*}
$\widebar{M}^{\widebar{\pi}_k}$ is an important operator which we will show is negative definite. It will create a negative drift that plays a significant role in establishing the convergence of $\|z_{i,k}\|^2$.


Note that the critic update \eqref{Alg:AC:critic_update} can be re-expressed in the vector form as
\begin{align*}
    \widehat{Q}_{i,k+1}=\widehat{Q}_{i,k}+\beta_k(R_i(O_k)+M(O_k)\widehat{Q}_{i,k}),
\end{align*}
which implies
\begin{align*}
    z_{i,k+1}-z_{i,k}=-(Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}})+\beta_k(R_i(O_k)+M(O_k)Q_i^{\widehat{\pi}_{k}}+M(O_k)z_{i,k}).
\end{align*}

Re-writing $\|z_{i,k+1}\|^2-\|z_{i,k}\|^2$
\begin{align}
    \|z_{i,k+1}\|^2-\|z_{i,k}\|^2&=2z_{i,k}^{\top}(z_{i,k+1}-z_{i,k})+\|z_{i,k+1}-z_{i,k}\|^2\notag\\
    &=2z_{i,k}^{\top}(z_{i,k+1}-z_{i,k}-\beta_k\widebar{M}^{\widehat{\pi}_{k}}z_{i,k})+\|z_{i,k+1}-z_{i,k}\|^2+2\beta_k z_{i,k}^{\top}\widebar{M}^{\widehat{\pi}_{k}}z_{i,k}\notag\\
    &=2\beta_k\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)-2z_{i,k}^{\top}(Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}})+\|z_{i,k+1}-z_{i,k}\|^2+2\beta_k z_{i,k}^{\top}\widebar{M}^{\widehat{\pi}_{k}}z_{i,k}
    \label{prop:conv_critic:eq1}
\end{align}



\begin{lem}\label{lem:hatpi_onestepdrift}
The error between $\widehat{\pi}_{k}$ and $\widehat{\pi}_{k+1}$ is bounded for all $k\geq 0$
\begin{align*}
    \|\widehat{\pi}_{k+1}-\widehat{\pi}_{k}\|\leq \frac{3(|\Scal||\Acal|)^{1/2} N \alpha}{\xi^{1/2}(1-\gamma)^{3/2}}.
\end{align*}
\end{lem}







\begin{lem}\label{lem:z_onestepdrift}
We have for all $i=0,\cdots,N$ and $k\geq 0$
\begin{align*}
    \|z_{i,k+1}-z_{i,k}\|^2\leq \frac{36 (|\Scal||\Acal|)^3 N^2 \beta^2}{\xi(1-\gamma)^7},\quad\text{and}\quad
    \|z_{i,k+1}-z_{i,k}\|\leq \frac{6 (|\Scal||\Acal|)^{3/2} N \beta}{\xi^{1/2}(1-\gamma)^{7/2}}.
\end{align*}
\end{lem}



\begin{lem}\label{lem:barM_negdef}
The matrix $\widebar{M}^{\widehat{\pi}_k}$ is negative definite for all $k\geq 0$
\begin{align*}
    x^{\top}\widebar{M}^{\widehat{\pi}_k}x\leq -\frac{(1-\gamma)\underline{\mu}\epsilon}{|\Acal|}\|x\|^2, \quad\forall x\in\mathbb{R}^{|\Scal||\Acal|},k\geq 0,
\end{align*}
where $\underline{\mu}=\min_{\pi,s}\mu_{\pi}(s)$, which is a positive constant due to the uniform ergodicity of the Markov chain under any policy.
(This is \citet{khodadadian2021finite}[Lemma 3].)
\end{lem}

\begin{lem}\label{lem:bound_Gamma}
Under Assumption \ref{assump:markov-chain}, we have for all $k\geq\tau$ and $i=0,\cdots,N$
\begin{align*}
    \mathbb{E}[\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)] \leq \frac{(3C_2+6C_3+4C_4) (|\Scal||\Acal|)^{3/2} N \beta\tau^2}{\xi^{1/2}(1-\gamma)^{7/2}},
\end{align*}
where $C_2=\frac{2\sqrt{2}|\Scal|^{3/2}|\Acal|^{3/2}}{(1-\gamma)^3}+\frac{8|\Scal|^2|\Acal|^3}{(1-\gamma)^2}\left(\left\lceil\log _{\rho} m^{-1}\right\rceil+\frac{1}{1-\rho}+2\right)$, $C_3=1+\frac{9\sqrt{2|\Scal||\Acal|}}{1-\gamma}$, and $C_4=\frac{4|\Scal|^{3/2}|\Acal|^{3/2}}{1-\gamma}(1+\frac{3|\Scal||\Acal|}{1-\gamma})$.
\end{lem}

Using the lemmas above in \eqref{prop:conv_critic:eq1}, we have for all $k\geq\tau$
\begin{align}
    \|z_{i,k+1}\|^2-\|z_{i,k}\|^2&=2\beta_k\Gamma_i(\widehat{\pi}_k,z_{i,k},O_k)-2z_{i,k}^{\top}(Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}})+\|z_{i,k+1}-z_{i,k}\|^2+2\beta_k z_{i,k}^{\top}\widebar{M}^{\widehat{\pi}_{k}}z_{i,k}\notag\\
    &\leq \frac{2(3C_2+6C_3+4C_4) (|\Scal||\Acal|)^{3/2} N \beta^2 \tau^2}{\xi^{1/2} (1-\gamma)^{7/2}} + 2\|z_{i,k}\|\|Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}}\|\notag\\
    &\hspace{20pt}+\frac{36 (|\Scal||\Acal|)^3 N^2 \beta^2}{\xi(1-\gamma)^7}-\frac{2(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2.
    \label{prop:conv_critic:eq2}
\end{align}

Using Lemma \ref{lem:Q_Lipschitz_pi} and \ref{lem:hatpi_onestepdrift}, we consider the second term of \eqref{prop:conv_critic:eq2}
\begin{align*}
    2\|z_{i,k}\|\|Q_i^{\widehat{\pi}_{k+1}}-Q_i^{\widehat{\pi}_{k}}\| &\leq \frac{2|\Scal||\Acal|}{(1-\gamma)^2}\|z_{i,k}\|\|\widehat{\pi}_{k+1}-\widehat{\pi}_{k}\|\leq \frac{6(|\Scal||\Acal|)^{3/2} N \alpha}{\xi^{1/2}(1-\gamma)^{7/2}}\|z_{i,k}\|\notag\\
     &\leq
     \frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2+
     \left(\frac{3(|\Scal||\Acal|)^{3/2} N \alpha}{\xi^{1/2}(1-\gamma)^{7/2}}\right)^2\frac{|\Acal|}{(1-\gamma)\underline{\mu}\epsilon\beta}\notag\\
     &\leq \frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2+
     \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta},
\end{align*}
where the third inequality follows from the fact that $2c\leq \frac{c^2}{d}+d$ for any scalar $c,d>0$. Plugging this bound back to \eqref{prop:conv_critic:eq2}, we have for all $k\geq\tau$
\begin{align*}
    \|z_{i,k+1}\|^2-\|z_{i,k}\|^2&\leq \frac{2(3C_2+6C_3+4C_4) (|\Scal||\Acal|)^{3/2} N \beta^2 \tau^2}{\xi^{1/2} (1-\gamma)^{7/2}}+\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2\notag\\
    &\hspace{20pt}+
    \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}+\frac{36 (|\Scal||\Acal|)^3 N^2 \beta^2}{\xi(1-\gamma)^7}-\frac{2(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2\notag\\
    &\leq -\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2 + C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta},
\end{align*}
where in the second inequality we re-combine the terms using $\tau\geq1$, $N\geq1$, and the definition of the constant $C_5=\frac{2(3C_2+6C_3+4C_4) (|\Scal||\Acal|)^{3/2} }{\xi^{1/2} (1-\gamma)^{7/2}}+\frac{36 (|\Scal||\Acal|)^3}{\xi(1-\gamma)^7}$.


Re-arranging this inequality, we have for all $k\geq\tau$
\begin{align}
    \frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2&\leq \|z_{i,k}\|^2-\|z_{i,k+1}\|^2 + C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}.
    \label{prop:conv_critic:eq3}
\end{align}

As a result,
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2&=\frac{1}{K}\sum_{k=0}^{\tau-1}\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2+\frac{1}{K}\sum_{k=\tau}^{K-1}\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2\notag\\
    &\leq \frac{1}{K}\sum_{k=0}^{\tau-1}\|z_{i,k}\|^2\hspace{-2pt}+\hspace{-2pt}\frac{1}{K}\sum_{k=\tau}^{K-1}(\|z_{i,k}\|^2-\|z_{i,k+1}\|^2)\hspace{-2pt}+\hspace{-2pt} \frac{1}{K}\sum_{k=\tau}^{K-1}\hspace{-2pt}\left(\hspace{-2pt}C_5 N^2 \beta^2\tau^2 \hspace{-2pt}+\hspace{-2pt} \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}\hspace{-2pt}\right)\notag\\
    &\leq\frac{1}{K}\sum_{k=0}^{\tau}\|z_{i,k}\|^2+C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta},
\end{align*}
where the second inequality follows from \eqref{prop:conv_critic:eq3} and the step size condition $\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\leq 1$.
Since $\|z_{i,k}\|^2=\|\widehat{Q}_{i,k}-Q_i^{\widehat{\pi}_k}\|^2\leq \frac{4|\Scal||\Acal|}{(1-\gamma)^2}$ for all $k\geq 0$, we can further simplify this inequality
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}\|z_{i,k}\|^2 & \leq\frac{1}{K}\sum_{k=0}^{\tau}\|z_{i,k}\|^2+C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}\notag\\
    &\leq\frac{4|\Scal||\Acal|(\tau+1)}{(1-\gamma)^2 K}+C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}.
\end{align*}


Dividing both sides of the inequality by $\frac{(1-\gamma)\underline{\mu}\epsilon\beta}{|\Acal|}$, we get
\begin{align*}
    \frac{1}{K}\sum_{k=0}^{K-1}\|z_{i,k}\|^2&\leq \frac{|\Acal|}{(1-\gamma)\underline{\mu}\epsilon\beta}\frac{8|\Scal||\Acal|\tau}{(1-\gamma)^2 K}+\frac{|\Acal|}{(1-\gamma)\underline{\mu}\epsilon\beta}\left(C_5 N^2 \beta^2\tau^2 + \frac{9|\Scal|^3|\Acal|^4 N^2 \alpha^2}{\xi\underline{\mu}(1-\gamma)^8\epsilon\beta}\right)\notag\\
    &\leq \frac{8|\Scal||\Acal|^2 \tau}{(1-\gamma)^3\underline{\mu}\epsilon\beta K}+\frac{C_5 N^2|\Acal|}{(1-\gamma)\underline{\mu}}\frac{\beta\tau^2}{\epsilon}+\frac{9|\Scal|^3|\Acal|^5 N^2 \alpha^2}{\xi\underline{\mu}^2 (1-\gamma)^9 \epsilon^2 \beta^2}
\end{align*}



\qed

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
